Durable Algorithms for Writable LL/SC and CAS with Dynamic Joining

We present durable implementations for two well known universal primitives -- CAS (compare-and-swap), and its ABA-free counter-part LLSC (load-linked, store-conditional). All our implementations are: writable, meaning they support a Write() operation; have constant time complexity per operation; allow for dynamic joining, meaning newly created processes (a.k.a. threads) of arbitrary names can join a protocol and access our implementations; and have adaptive space complexities, meaning the space use scales in the number of processes $n$ that actually use the objects, as opposed to previous protocols which are designed for a maximum number of processes $N$. Our durable Writable-CAS implementation, DuraCAS, requires $O(m + n)$ space to support $m$ objects that get accessed by $n$ processes, improving on the state-of-the-art $O(m + N^2)$. By definition, LLSC objects must store "contexts" in addition to object values. Our Writable-LLSC implementation, DuraLL, requires $O(m + n + C)$ space, where $C$ is the number of "contexts" stored across all the objects. While LLSC has an advantage over CAS due to being ABA-free, the object definition seems to require additional space usage. To address this trade-off, we define an External Context (EC) variant of LLSC. Our EC Writable-LLSC implementation is ABA-free and has a space complexity of just $O(m + n)$. To our knowledge, we are the first to present durable CAS algorithms that allow for dynamic joining, and our algorithms are the first to exhibit adaptive space complexities. To our knowledge, we are the first to implement any type of durable LLSC objects.

==> Model-Formal.tex <==
\section{Model}
 
In this section, we describe our model for processes and memory, and what it means to implement standard objects, durable objects, or detectable durable objects.

\subsection{Processes}

We assume that processes are asynchronous.
A process may {\em crash} at any time and {\em restart} at any subsequent time.
A process may crash and restart an arbitrary number of times.
When a process $p$ crashes, the contents of all its internal registers, including its program counter, lose their contents, i.e., they are set to arbitrary values.
When $p$ restarts, its program counter is reset to some pre-determined memory address, about which we make no assumption.

\subsection{Memory}

We assume that memory is {\em persistent} and supports {\em atomic} read and CAS operations.
Persistence means that the memory contents are unaffected by process crashes.
Atomicity means that a read or a CAS operation on a memory word executes instantly.
If $X$ is a memory word and $old$ and $new$ are values (in process' registers), {\em read}$(X)$ returns $X$'s value and {\em CAS}$(X, old, new)$ behaves as follows: if $X$'s value is $old$, $X$'s value changes to $new$ and {\em true} is returned; otherwise, $X$'s value is unchanged and {\em false} is returned.

\subsection{Type}

A {\em type} is specified by a set of states $\Sigma$; a set of operations $OP$;
for each $op \in OP$, a set of arguments $ARG(op)$ and a set of responses $RES(op)$;
a {\em state transition function} $\delta$ and a {\em response function} $\hat{\delta}$ such that, if $\sigma \in \Sigma$, $op \in OP$, $args \in ARG(OP)$, then $\delta(\sigma, op(args)) \in \Sigma$ and $\hat{\delta}(\sigma, op, args) \in RES(op)$.
We illustrate this definition with three types, which are of interest in this paper.

\begin{itemize}
\item
\underline{Writable CAS}:
The type {\bf Writable CAS} with value set $V$ is defined by:
\begin{itemize}
\item
$\Sigma = V$
\item
$OP = \{\mbox{read}, \mbox{write}, \mbox{CAS} \}$
\item
$ARG(\mbox{read}) = \emptyset$, $ARG(\mbox{write}) = V$, and $ARG(\mbox{CAS}) = V \times V$.
\item
$RES(\mbox{read}) = V$, $RES(\mbox{write}) = \{ack\}$, and
$RES(\mbox{CAS}) = \{\mbox{\em true}, \mbox{\em false}\}$.
\item
$\delta(\sigma, \mbox{\em read}()) = \sigma \,$; 
$\; \; \delta(\sigma, \mbox{\em write}(v)) = v\,$;
$\; \; \delta(\sigma, \mbox{\em CAS}(old, new)) = new \mbox{ if $\sigma = old$, and $\sigma$ otherwise}$.
\item
$\hat{\delta}(\sigma, \mbox{\em read}()) = \sigma \,$; 
$\; \; \hat{\delta}(\sigma, \mbox{\em write}(v)) = ack \,$; 
$\; \; \hat{\delta}(\sigma, \mbox{\em CAS}(old, new)) = \mbox{\em true} \mbox{ if $\sigma = old$, and $\,$ {\em false} otherwise}$.
\end{itemize}

\item
\underline{Writable LL/SC}:
Informally, an LL/SC object supports LL and SC operations, and its state consists of a context and a value. When a process performs LL or SC, it supplies an ID as the first argument. If LL$(p)$ is invoked when the object's value and context are $v$ and $c$, the object returns $v$ and remembers that $c$ is the context last seen by $p$. When SC$(p, v')$ is invoked, the operation checks the object's current context against the last context seen by $p$. If they are equal, the object's value is set to $v'$, the object's context is set to a value that is different from all earlier contexts, and {\em true} is returned. Otherwise, the SC operation returns {\em false}, without affecting the object's state.
Formally, the type {\bf Writable LL/SC with value set $V$ and ID set $ID$} is defined by:
\begin{itemize}
\item
$\Sigma = \{(c, v, last) \mid c \in \N, v \in V, last:ID \rightarrow \N \}$, where $\N$ is the set of natural numbers
\item
$OP = \{\mbox{LL}, \mbox{SC}, \mbox{write}, \mbox{VL} \}$
\item
$ARG(\mbox{LL}) = ARG(\mbox{VL}) = ID$, and $ARG(\mbox{SC}) = ARG(\mbox{write}) = ID \times V $.
\item
$RES(\mbox{LL}) = V$, $RES(\mbox{write}) = \{ack\}$, and
$RES(\mbox{SC}) = RES(\mbox{VL}) = \{\mbox{\em true}, \mbox{\em false}\}$.
\item
$\delta((c, v, f), \mbox{\em LL}(p)) = (c,v,f')$, where $f'$ coincides with $f$ except at $p$, where $f'(p) = c$

$\delta((c, v, f), \mbox{\em SC}(p, v')) = 
\left\{
     \begin{array}{lr}
       (c+1, v', f) \; \; \text{ if $f(p) = c$} \\
       (c, v, f) \; \; \text{ otherwise} \\
     \end{array}
   \right. $

$\delta((c, v, f), \mbox{\em VL}(p)) = (c,v,f)$

$\delta((c, v, f), \mbox{\em write}(p, v')) = (c+1,v',f)$

\item
$\hat{\delta}((c, v, f), \mbox{\em LL}(p)) = v$

$\hat{\delta}((c, v, f), \mbox{\em SC}(p, v')) = \hat{\delta}((c, v, f), \mbox{\em VL}(p)) = 
\left\{
     \begin{array}{lr}
       \mbox{\em true} \; \; \text{ if $f(p) = c$} \\
       \mbox{\em false} \; \; \text{ otherwise} \\
     \end{array}
   \right. $

$\hat{\delta}((c, v, f), \mbox{\em write}(p, v')) = \mbox{\em ack}$
\end{itemize}

\item
\underline{Writable External Context LL/SC}:
For designing the algorithms of this paper, we have found it useful to define an ``External Context'' version of the LL/SC type, where the burden of remembering the last seen context of each ID is shifted from the object to the invoking process.
Thus, when a process $p$ invokes ECLL, the object simply returns the current context $c$ (along with the current value), and won't bother to remember $c$ as the last seen context of $p$.
When a process invokes SC, it passes a context $c'$ as an additional argument; the object checks the supplied context $c'$ against its current context and changes state if and only if the two contexts are the same.
Formally, the type {\bf Writable External Context LL/SC with value set $V$} is defined by:
\begin{itemize}
\item
$\Sigma = \N \times V$, where $\N$ is the set of natural numbers.
\item
$OP = \{\mbox{ECLL}, \mbox{ECSC}, \mbox{write}, \mbox{ECVL} \}$
\item
$ARG(\mbox{ECLL}) = ARG(\mbox{ECVL}) = \N$, $ARG(\mbox{SC}) = \N \times V$, and $ARG(\mbox{write}) = V$.
\item
$RES(\mbox{ECLL}) = \N \times V$, $RES(\mbox{write}) = \{ack\}$, and
$RES(\mbox{ECSC}) = RES(\mbox{ECVL}) = \{\mbox{\em true}, \mbox{\em false}\}$.
\item
$\delta((c, v), \mbox{\em ECLL}()) = (c,v)$

$\delta((c, v), \mbox{\em ECSC}(c', v')) = 
\left\{
     \begin{array}{lr}
       (c+1, v') \; \; \text{ if $c' = c$} \\
       (c, v) \; \; \text{ otherwise} \\
     \end{array}
   \right. $

$\delta((c, v), \mbox{\em ECVL}()) = (c,v)$

$\delta((c, v), \mbox{\em write}(v')) = (c+1,v')$

\item
$\hat{\delta}((c, v), \mbox{\em ECLL}()) = (c,v)$

$\hat{\delta}((c, v), \mbox{\em ECSC}(c', v')) = \hat{\delta}((c, v), \mbox{\em ECVL}(c')) = 
\left\{
     \begin{array}{lr}
       \mbox{\em true} \; \; \text{ if $c' = c$} \\
       \mbox{\em false} \; \; \text{ otherwise} \\
     \end{array}
   \right. $

$\hat{\delta}((c, v), \mbox{\em write}(v')) = \mbox{\em ack}$
\end{itemize}

\end{itemize}

\subsection{Non-Durable Objects}

A {\em non-durable object} has a type and a state.
The object's type is fixed, but its state may change over time.
In the following, let $\mathcal O$ be an object of type $T$.
For each $op \in T.OP$, $\mathcal O$ provides a method $op(\mbox{\tt Proc-Info } p, \, \mbox{\tt Args } arg)$, where the second parameter $arg \in ARG(op)$ is the operation's argument, and the first parameter $p$ has traditionally been the caller's process ID.
In this work, $p$ is the caller's ``created ID'' instead of the real ID.
More specifically, for each type $T$, we provide a method named {\sc CreateHandle}$()$, which a process $\pi$ calls and uses its return value (a memory address that we call {\em handle}) from then on as its created ID.
Thus, the method for operation $op$ has the signature $op(\mbox{\tt Handle } h, \, \mbox{\tt Args } arg)$.
Once a process creates a handle $h$, it can use that same handle $h$ for accessing any number of type $T$ objects.
Furthermore, a process $\pi$ can call {\sc CreateHandle}$()$ multiple times to create for itself multiple identities---a feature that is sometimes useful, as we will see.

If $\alpha$ is an execution of ${\mathcal O}.op(h,arg)$ by a process $\pi$, we say $\alpha$ is an {\em operation execution}, or simply an {\em operation}, of $op$ on $\mathcal O$ by $\pi$ with handle $h$ and argument $arg$.
The operation {\em completes} (if and) when the method returns, and the return value is $\mathcal O$'s {\em response} to the operation.
When accessing non-durable objects, processes are required to obey the following rule, which states that there cannot be more than one pending operation with the same handle.

\begin{definition}\label{ndc}
{\em 
\underline{Non-Durable Objects Contract}:
For all non-durable objects $\mathcal O$ and all handles $h$:
\begin{enumerate}
\item
After starting an operation $\alpha$ with a handle $h$, no other operation is started with the handle $h$ until $\alpha$ completes.
\item
If a process $\pi$ starts an operation ${\mathcal O}.op(h,arg)$ and crashes at some time $t$ before the operation completes, then no operation is started after $t$ with handle $h$. (Thus, even after a crashed process restarts, it does not pursue its crashed operation, so a crashed operation never completes.)
\end{enumerate}
}
\end{definition}

The consistency property required of non-durable objects is {\em linearizability} \cite{}, which states that every completed operation takes effect instantaneously at some time during the interval of its execution, and every incomplete operation either does not take effect or takes effect instantaneously at some time after its start. More precisely:

\begin{definition}\label{ndcons}
{\em 
\underline{Non-Durable Linearizability}: 
For all non-durable objects $\mathcal O$ and all handles $h$:
\begin{enumerate}
\item
If an operation ${\mathcal O}.op(h,arg)$ starts at $t$ and completes at $t'$, then it linearizes at some time $\tau$ during the interval from $t$ to $t'$, i.e., if $\sigma$ is $\mathcal O$'s state at $\tau$, $\delta(\sigma, op(arg))$ is $\mathcal O$'s state immediately after $\tau$, and the operation returns $\hat{\delta}(\sigma, op(arg))$ when it completes at $t'$.
\item
If an operation ${\mathcal O}.op(h,arg)$ starts at $t$ and is incomplete, either it does not linearize or it linearizes at some time $\tau \ge t$.
If the operation does not linearize, it does not affect $\mathcal O$'s state.
Otherwise, if if $\sigma$ is $\mathcal O$'s state at $\tau$, $\delta(\sigma, op(arg))$ is $\mathcal O$'s state immediately after $\tau$.
\end{enumerate}
}
\end{definition}

Finally, the correctness condition states that non-durable objects guarantee linearizable behavior provided that they are used properly.

\begin{definition}\label{ndcorr}
{\em 
\underline{Non-Durable Objects Correctness}: If Non-Durable Objects Contract is met, then Non-Durable Linearizability is guaranteed.
}
\end{definition}

\subsection{Durable objects}


==> TypeSpecs.tex <==
\section{Specifications of the ABA-free objects implemented}

Each object has a {\em type}, which specifies the set $\Sigma$ of possible states of the object, the set $OP$ of operations that can be executed on the object, the set $RES$ of possible responses to operations, and a transition relation $\delta$ from $\Sigma \times OP$ to $\Sigma \times RES$. If $(\sigma', r) \in \delta(\sigma, op)$, it means that if the operation $op$ is executed when the object is in the state $\sigma$, the object may change its state to $\sigma'$ and return the response $r$.
The relation $\delta$ is the object's {\em sequential specification}, and the object is {\em deterministic} if $\delta$ is a function.
The following are the types of objects studied in this paper.

\subsection{ECW type}

For the {\em Writable External Context LL/SC} type, henceforth {\em ECW}, each state $\sigma$ is a pair $(\sigma.\seq, \sigma.\val)$ of integers. 
We call $\sigma.\seq$ and $\sigma.\val$ the object's {\em sequence number} and {\em value} in the state $\sigma$.
The operations are $\CLL{}$, $\CSC{\s,\v}$, $\CVL{\s}$, and $\Write{\v}$, where the arguments $\s$ and $\v$ are integers.
The sequential specification is as follows.
\begin{itemize}
\item
$\CLL{}$, when executed in state $\sigma$, leaves the state unchanged and return $\sigma$.
\item
$\CSC{\s, \v}$, when executed in state $\sigma$, leaves the state unchanged and returns $\false$ if $\sigma.\seq \neq \s$; otherwise, returns $\true$ and changes the state to $(s',v)$, where $s'$ is any integer greater than $\sigma.\seq$.
\item
$\CVL{\s}$, when executed in state $\sigma$, returns the Boolean $\s = \sigma.\seq$.
\item
$\Write{\v}$, when executed in state $\sigma$, returns $\true$ and changes the state to $(s', \v)$, where $s'$ is any integer greater than $\s$.
\end{itemize}

\subsection{EC type}

The {\em Non-Writable External Context LL/SC} type, henceforth {\em EC}, is the ECW type without the $\Write$ operation.

\subsection{Writable LL/SC type}

LL/SC objects are similar to External Context LL/SC objects, but they don't exchange sequence numbers with processes; instead, each object stores, for each process $\pi$, the latest sequence number that $\pi$'s LL has seen. 
Specifically, an object's state $\sigma$ consists of $\sigma.\seq$, $\sigma.\val$, and $\sigma.\last(\pi)$, for each process $\pi$.
$\CLL{p}$ returns $\sigma.\val$ and stores $\sigma.\seq$ in $\sigma.\last(\pi)$.
$\CSC{\pi, \s, \v}$ leaves the state unchanged and returns $\false$ if $\sigma.\seq \neq \s$; otherwise, returns $\true$, and sets $\sigma.\val$ to $\v$, and $\sigma.\seq$ to any integer greater than $\s$.
$\CVL{\pi}$ returns the Boolean $\sigma.\last(\pi) = \sigma.\seq$.
$\Write(\pi, \v)$ returns $\true$, and sets $\sigma.\val$ to $\v$, and $\sigma.\seq$ to any integer greater than $\s$.



   



==> alg/DurEC-Annotated.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm*}
\caption{: The \annotate{Annotated} $\DurEC$ class for Detectable, Durable, External Context LL/SC objects.}
\label{alg:DurEC-Annotated}
\begin{algorithmic}[1]

\medskip 

\Statex \cmdclass $\DurEC$:

\medskip 

\Statex \tab \cmdinstancevar \; (\Thandle, \Tint) \: $\X$ \Comment{$X$ is a pair $(\X.\hndl, \X.\seq)$ stored in NVM}
\Statex \tab \cmdinstancevar \; (\Tint, \Tint) \: $\Y$ \Comment{$Y$ is a pair $(\Y.\seq, \Y.\val)$ stored in NVM}

\medskip 

\Statex \tab \cmdstruct $\textit{handle} \:\{$
\Statex \tab[2] $\Tint \: \Last$
\Statex \tab[2] $\Tint \: \Val$
\Statex \tab $\}$

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\CreateHandle{}$
\State \tab[2] $\cmdreturn \: \cmdnew \: handle \{\Last = 0\}$ \Comment{fields $\Last$ and $\Val$ are stored in NVM; $\Val$ is arbitrarily initialized}

\medskip 

\Statex \tab \cmdconstructor $\DurEC(\Tint\: \initval)$
\State \tab[2] $\X \gets (null, 0)$
\State \tab[2] $\Y \gets (0, \initval)$

\medskip 

\Statex \tab \cmdprocedure $\CLL{\Thandle\: \h}$
\State \tab[2] \cmdreturn $\Y$

\medskip 

\Statex \tab \cmdprocedure $\CVL{\Thandle\: \h, \Tint \: \s}$
\State \tab[2] \cmdreturn $\Y.\seq = \s$

\medskip 

\Statex \tab \cmdprocedure $\CSC{\Thandle\: \h, \Tint \: \s, \Tint \: \v}$
\Statex \tab \annotate{\underline{$\h.\args \gets (\s, \v); \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \h.\Last$}}

\State \tab[2] \cmdif $\Y.\seq \ne \s$ \cmdthen \{\cmdreturn $\false$; \annotate{\underline{$\h.\args \gets \bot; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \bot$}}\}

\State \tab[2] $\h.\Val \gets \v$
\State \tab[2] $\hh \gets \X.\hndl$ %; \cmdif $\x.\seq \ne \s$ \cmdthen \cmdreturn $\false$
\State \tab[2] $\sh \gets \max(\h.\Last, \s) + 1$
\State \tab[2] $\ret \gets \CAS{\X, (\hh, \s), (\h, \sh)}$
\State \tab[2] $\forward{\h}$
\State \tab[2] \cmdreturn $\ret$ 
\Statex \tab[2] \annotate{\underline{$\h.\args \gets \bot; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \bot$}}

\medskip 

\Statex \tab \cmdprocedure $\forward{\Thandle\: \h}$
% Update Last
\State \tab[2] $\x \gets \X$ 
\State \tab[2] $\sh \gets \x.\hndl.\Last$ 
\State \tab[2] \cmdif $\sh < \x.\seq$ \cmdthen $\CAS{\x.\hndl.\Last, \sh, \x.\seq}$

% Push X to Y
\State \tab[2] $\vh \gets \x.\hndl.\Val$ 
\State \tab[2] $\y \gets \Y$
\State \tab[2] \cmdif $\y.\seq < \x.\seq$ \cmdthen $\CAS{\Y, \y, (\x.\seq, \vh)}$

\annotate{
\Statex \tab[2] \underline{\cmdif CAS is successful \cmdthen}
\Statex \tab[3] \underline{$(\objstate.\seq, \objstate.\val) \gets (x.seq, \vh)$}
\Statex \tab[3] \underline{$\X.\hndl.\linearized \gets \true$}
\Statex \tab[3] \underline{$\X.\hndl.\visible \gets \true$}
\Statex \tab[3] \underline{$\forall \hh, \cmdif\: \hh.\pc \in \{7,8,9,10,11.*\} \wedge \neg \hh.\linearized \:\cmdthen\: \hh.\linearized \gets \true$}
}

\State \tab[2] \cmdreturn

\medskip 

\Statex \tab \cmdprocedure $\Recover{\Thandle\: \h}$ 
\State \tab[2] $\forward{\h}$
\State \tab[2] \cmdreturn
\Statex \tab[2] \annotate{\underline{$\h.\args \gets \bot; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \bot$}}

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\Detect{\Thandle\: \h}$
\State \tab[2] \cmdreturn $\h.\Last$


\end{algorithmic}
\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> alg/DurECW-Annotated.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm*}
\caption{
The \annotate{Annotated} DurECW class - Supports ECLL, ECVL, ECSC and Write operations 
}
\label{alg:DurECW-Annotated}

% \begin{footnotesize}
\begin{algorithmic}[1]

\Statex \cmdclass \DurECW:

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\CreateHandle{}$
\State \tab[2] \cmdreturn  $\textbf{handle}$ \{$\Critical \gets \text{DurEC}.\CreateHandle{},$
$\Casual \gets \text{DurEC}.\CreateHandle{} \} $
%$\contexts \gets \{\}\}$

\medskip 

\Statex \tab \cmdprocedure $\DurECW(\initval)$
\State \tab[2] $\W \gets \ECL{(0, 0)}$ 
\State \tab[2] $\Z \gets \ECL{(\initval, 0)}$
\Statex \tab[2] \annotate{\underline{$\installer \gets \bot$}}

\medskip 

\Statex \tab \cmdprocedure $\CLL{\Thandle\: \h}$
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$; \cmdreturn $(\z.\seq, \z.\val)$

\medskip 

\Statex \tab \cmdprocedure $\CVL{\Thandle\: \h, \Tint \: \s}$
\State \tab[2] \cmdreturn $\Z.\CVL{\h.\Casual, \s}$

\medskip 

\Statex \tab \cmdprocedure $\CSC{\Thandle\: \h, \Tint \: \s, \Tint \: \v}$
\Statex \tab \annotate{\underline{$\h.\op \gets \Rcas{\old, \new}; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \DurEC.\Detect{\h.\Critical}$}}
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$; \cmdif $\s \ne \z.\seq$ \cmdreturn $\false$
\State \tab[2] $\transfer{\h}$
\State \tab[2] $\ret \gets \Z.\CSC{\h.\Critical, \s, (\v, \z.\bit)}$
\annotate{
\Statex \tab[2] \underline{$\linearized \gets \true$; $\response \gets \ret$}
\Statex \tab[2] \underline{\cmdif ECSC is successful \cmdthen \{$\visible \gets \true$; $\objstate \gets \Z$}\}
}
\State \tab[2] \cmdreturn $r$
\Statex

\Statex \tab \cmdprocedure $\Write{\Thandle\: \h, \Tint \: \v}$
\Statex \tab \annotate{\underline{$\h.\op \gets \Write{\v}; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \DurEC.\Detect{\h.\Critical}$}}
\State \tab[2] $\w \gets \W.\CLL{\h.\Casual}$ 
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$
\State \tab[2] \cmdif $\z.\bit = \w.\bit$ \cmdthen $\W.\CSC{\h.\Critical, \w.\seq, (\v, 1 - \w.\bit)}$ \annotate{\underline{; \cmdif ECSC is successful \cmdthen $\installer \gets \h$}}
\State \tab[2] $\transfer{\h}$
\State \tab[2] $\transfer{\h}$
\State \tab[2] \cmdreturn $\true$

\medskip 

\Statex \tab \cmdprocedure $\transfer{\Thandle \: \h}$
\State \tab[2] $\zh \gets \Z.\CLL{\h.\Casual}$
\State \tab[2] $\wh \gets \W.\CLL{\h.\Casual}$
\State \tab[2] \cmdif $\zh.\bit \neq \wh.\bit$ \cmdthen $\Z.\CSC{\h.\Casual, \zh.\seq, (\wh.\val, \wh.\bit)}$
\annotate{
\Statex \tab[2] \underline{\cmdif ECSC is successful \cmdthen}
\Statex \tab[3] \underline{$\installer.\linearized \gets \true$; $\installer.\response \gets ack$; $\installer.\visible \gets \true$}
\Statex \tab[3] \underline{$\objstate \gets \Z$}
\Statex \tab[3] \underline{$\installer \gets \bot$}
\Statex \tab[3] \underline{for all handles $g$ such that $\neg g.\linearized \wedge (g.\pc \in \{12, 13.*, 14.*\} \vee (g.\pc = 11 \wedge (\wh \neq \W))) $}:
\Statex \tab[4] \underline{$g.\linearized \gets \true$; $g.\response \gets \true$}
}

\medskip 

\Statex \tab \cmdprocedure $\Recover{\Thandle \: \h}$
\State \tab[2] $\W.\Recover{\h.\Critical}$
\State \tab[2] $\Z.\Recover{\h.\Critical}$
\State \tab[2] $\W.\Recover{\h.\Casual}$
\State \tab[2] $\Z.\Recover{\h.\Casual}$
\State \tab[2] $\transfer{\h}$
\State \tab[2] $\transfer{\h}$

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\Detect{\textbf{handle*} \: \h}$
\State \tab[2] \cmdreturn $(\textsc{DurEC}.\Detect{\h.\Critical}, \true)$

\end{algorithmic}
% \end{footnotesize}


\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> alg/DuraCAS-Annotated.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm*}
\caption{
The \annotate{Annotated} DuraCAS class - Supports Read, CAS, Write operations 
}
\label{alg:DuraCAS-Annotated}

% \begin{footnotesize}
\begin{algorithmic}[1]

\Statex \cmdclass \DuraCAS:

% \medskip 

% \Statex \tab \cmdinstancevar \; \textbf{DurEC} \: $\W$ 
% \Comment{$\W$ holds a pair $(\W.\seq, (\W.\val, \W.\bit))$}
% \Statex \tab \cmdinstancevar \; \textbf{DurEC} \: $\Z$ 
% \Comment{$\Z$ holds a pair $(\Z.\seq, (\Z.\val, \Z.\bit))$} 

% \medskip 

% \Statex \tab $\cmdstruct \: \textit{handle} \:\{$
% \Statex \tab[2] $\textbf{DurEC}.\Thandle \: \Critical$
% \Statex \tab[2] $\textbf{DurEC}.\Thandle \: \Casual$
% %\Statex \tab[2] $\textbf{String} \: \mbox{op}$
% \Statex \tab $\}$

\medskip 


\Statex \tab \cmdstatic \cmdprocedure $\CreateHandle{}$
\State \tab[2] \cmdreturn \cmdnew 
$handle \{
\Critical \gets \DurEC.\CreateHandle{},  
\Casual \gets \DurEC.\CreateHandle{}
%,op \gets \bot
\}$

\medskip 

\Statex \tab \cmdprocedure $\DuraCAS(\Tint \: \initval)$
\State \tab[2] $\W \gets \ECL{(0, 0)}$ 
\State \tab[2] $\Z \gets \ECL{(\initval, 0)}$
\Statex \tab[2] \annotate{\underline{$\installer \gets \bot$}}


\medskip 

\Statex \tab \cmdprocedure $\Read{\Thandle \: \h}$
\Statex \tab \annotate{\underline{$\h.\op \gets \Read{}; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \DurEC.\Detect{\h.\Critical}$}}
%\State \tab[2] $\h.op \gets \mbox{Read}$
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$
\State \tab[2] \cmdreturn $\z.\val$


\medskip 

\Statex \tab \cmdprocedure $\Rcas{\Thandle \: \h, \Tint \: \old, \Tint \: \new}$
\Statex \tab \annotate{\underline{$\h.\op \gets \Rcas{\old, \new}; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \DurEC.\Detect{\h.\Critical}$}}
%\State \tab[2] $\h.op \gets \mbox{CAS}$
\State \tab[2] \cmdfor $i \gets 1 \mbox{ to } 2$
\State \tab[3] $\z \gets \Z.\CLL{\h.\Casual}$ 
\Statex \tab[3] \annotate{\underline{\cmdif $\z.val \neq \old$ \cmdthen $(\linearized, \response) \gets (\true, \false)$ \cmdelse \cmdif $old = new$ \cmdthen $(\linearized, \response) \gets (\true, \true)$}}
\State \tab[3] \cmdif $\z.\val \ne \old$ \cmdthen \cmdreturn $\false$
\State \tab[3] \cmdif $\old = \new$ \cmdthen \cmdreturn $\true$
\State \tab[3] $\transfer{\h}$
\State \tab[3] \cmdif $\Z.\CSC{\h.\Critical, \z.\seq, (\new, \z.bit)}$ \cmdthen

\annotate{
\Statex \tab[3] \underline{\cmdif ECSC is successful \cmdthen}
\Statex \tab[4] \underline{$\linearized \gets \true$; $\visible \gets \true$}
\Statex \tab[4] \underline{$(\objstate, \response) \gets \delta(\objstate, \cas(\old, \new))$}
\Statex \tab[4] \underline{for all handles $g$ such that $\neg g.\linearized \wedge g.\pc \in \{6, 7, 8, 9, 10.*, 11\}$}
\Statex \tab[5] \underline{$g.\linearized \gets \true$; $g.\response \gets \false$}
}

\State \tab[4] \cmdreturn $\true$
\State \tab[2] \cmdreturn $\false$

\medskip 

\Statex \tab \cmdprocedure $\Write{\Thandle \: \h,\Tint \: \v}$
\Statex \tab \annotate{\underline{$\h.\op \gets \Write{\v}; \h.\linearized \gets \false; \h.\visible \gets \false; \h.\detval \gets \DurEC.\Detect{\h.\Critical}$}}
%\State \tab[2] $\h.op \gets \mbox{Write}$
\State \tab[2] $\w \gets \W.\CLL{\h.\Casual}$ 
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$ \annotate{; \underline{\cmdif $\z.val = \v$ \cmdthen $\linearized \gets \true$}}
\State \tab[2] \cmdif $\z.\val = \v$ \cmdthen \cmdreturn $ack$
\State \tab[2] \cmdif $\z.\bit = \w.\bit$ \cmdthen $\W.\CSC{\h.\Critical, \w.\seq, (\v, 1 - \w.\bit)}$ \annotate{\underline{; \cmdif ECSC is successful \cmdthen $\installer \gets \h$}}
\State \tab[2] $\transfer{\h}$ 
\State \tab[2] $\transfer{\h}$ 
\State \tab[2] \cmdreturn $ack$

\medskip 

\Statex \tab \cmdprocedure $\transfer{\Thandle \: \h}$
\State \tab[2] $\zh \gets \Z.\CLL{\h.\Casual}$
\State \tab[2] $\wh \gets \W.\CLL{\h.\Casual}$
\State \tab[2] \cmdif $\zh.\bit \neq \wh.\bit$ \cmdthen 
\Statex \tab[3] $\Z.\CSC{\h.\Casual, \zh.\seq, (\wh.\val, \wh.\bit)}$
\annotate{
\Statex \tab[3] \underline{\cmdif ECSC is successful \cmdthen}
\Statex \tab[4] \underline{$\installer.\linearized \gets \true$; $\installer.\response \gets ack$; $\installer.\visible \gets \true$}
\Statex \tab[4] \underline{$\objstate \gets \installer.args$}
\Statex \tab[4] \underline{$\installer \gets \bot$}
\Statex \tab[4] \underline{for all handles $g$ such that $\neg g.\linearized \wedge g.\pc \in \{18.*, 19.*\}$:}
\Statex \tab[5] \underline{$g.\linearized \gets \true$; $g.\response \gets ack$}
\Statex \tab[4] \underline{for all handles $g$ such that $\neg g.\linearized \wedge (g.\pc \in \{6,7, 8, 9, 10.*, 11\} \wedge (g.\old \neq \Z.val))$:}
\Statex \tab[5] \underline{$g.\linearized \gets \true$; $g.\response \gets \false$}
}

% \Statex \tab \cmdprocedure $\transfer{\Thandle \: \h}$
% \State \tab[2] $\w \gets \W.\CLL{\h.\Casual}$
% \State \tab[2] \cmdfor $i \gets 1 \mbox{ to } 2$
% \State \tab[3] $\z \gets \Z.\CLL{\h.\Casual}$
% \State \tab[3] \cmdif $\z.\bit \neq \w.\bit \wedge \W.\CVL{\h.\Casual, \w.\seq}$
% \State \tab[4] \cmdif $\Z.\CSC{\h.\Casual, \x.\seq, (\w.\val, \w.\bit)}$ \cmdreturn
% \State \tab[2] \cmdreturn

\medskip 

\Statex \tab \cmdprocedure $\Recover{\Thandle \: \h}$
\State \tab[2] $\W.\Recover{\h.\Critical}$
\State \tab[2] $\Z.\Recover{\h.\Critical}$
\State \tab[2] $\W.\Recover{\h.\Casual}$
\State \tab[2] $\Z.\Recover{\h.\Casual}$
%\State \tab[2] \cmdif $\h.op = \mbox{CAS}$ \cmdthen $\Z.\Recover{\h.\Critical}$
%\State \tab[2] \cmdif $\h.op = \mbox{Write}$:
%\State \tab[3] $\W.\Recover{\h.\Critical}$
\State \tab[2] $\transfer{\h}$
\State \tab[2] $\transfer{\h}$

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\Detect{\Thandle \: \h}$
\State \tab[2] \cmdreturn $(\textsc{DurEC}.\Detect{\h.\Critical}, \true)$
%\State \tab[2] $c \gets \textsc{DurEC}.\Detect{\h.\Critical}$
%\State \tab[2] \cmdif $\h.op = CAS$ \cmdthen \cmdreturn $(c, \true)$ \cmdelse \cmdreturn $(c, ack)$

%\State \tab[2] \cmdif $\h.op = Write$ \cmdthen \cmdreturn $(c, ack)$

\end{algorithmic}
% \end{footnotesize}


\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> alg/DuraLL-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm*}
\caption{
The DuraLL class - Supports LL, VL, SC and Write operations 
}
\label{alg:LLSC-Write}

% \begin{footnotesize}
\begin{algorithmic}[1]

\Statex \cmdclass \DuraLL:

\medskip 

\Statex \tab \textbf{instance variable} \; \textbf{DurEC} \: $\W$ 
\Comment{$\W$ holds a pair $(\W.seq, (\W.\val, \W.\bit))$}
\Statex \tab \textbf{instance variable} \; \textbf{DurEC} \: $\Z$ 
\Comment{$\Z$ holds a pair $(\Z.seq, (\Z.\val, \Z.\bit))$}

\medskip 

\Statex \tab $\textbf{struct} \: \textit{handle} \:\{$
\Statex \tab[2] $\textbf{DurEC.handle} \: \Critical$
\Statex \tab[2] $\textbf{DurEC.handle} \: \Casual$
\Statex \tab[2] $\textbf{HashMap} \: (\textbf{DuraLL} \rightarrow \textbf{int})  \: \mbox{contexts}$
\Statex \tab $\}$

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\CreateHandle{}$
\State \tab[2] \cmdreturn  $\textbf{handle}$ \{ 
$\Critical \gets \text{DurEC}.\CreateHandle{},$
$\Casual \gets \text{DurEC}.\CreateHandle{} \} $
%$\contexts \gets \{\}\}$

\medskip 

\Statex \tab \cmdprocedure $\DuraLL(\textit{init\_val})$
\State \tab[2] $\W \gets \ECL{(0, 0)}$ 
\State \tab[2] $\Z \gets \ECL{(init\_val, 0)}$

\medskip 

\Statex \tab \cmdprocedure $\LL{\textbf{handle*} \: \h}$
\State \tab[2] $\z \gets \Z.\CLL{\h.\Critical}$
\State \tab[2] $\h.\contexts(\self) \gets \z.\seq$
\State \tab[2] \cmdreturn $\z.\val$

\medskip 

\Statex \tab \cmdprocedure $\VL{\textbf{handle*} \: \h}$
\State \tab[2] \cmdif $\self$ not in $\h.\contexts.keys$ \cmdthen \cmdreturn $false$
\State \tab[2] \cmdreturn $\Z.\CLL{\h.\Critical}.\seq = \h.\contexts(seq)$

\medskip 

\Statex \tab \cmdprocedure $\SC{\textbf{handle*} \: \h, \textbf{int} \: \val}$
\State \tab[2] \cmdif $\self$ not in $\h.\contexts.keys$ \cmdthen \cmdreturn $false$
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$
\State \tab[2] $\seq \gets \h.\contexts(self)$
\State \tab[2] \cmdif $\z.\seq \ne \seq$ \cmdthen \cmdreturn $\false$ 
\State \tab[2] $\transfer{\h.\Casual}$
\State \tab[2] \cmdreturn $\Z.\CSC{\h.\Critical, \seq, \val}$

\medskip 

\Statex \tab \cmdprocedure $\Write{\textbf{handle*} \: \h,\textbf{int} \: \new}$
\State \tab[2] $\w \gets \W.\CLL{\h.\Casual}$ 
\State \tab[2] $\z \gets \Z.\CLL{\h.\Casual}$
\State \tab[2] \cmdif $\z.\val = \new$ \cmdreturn
\State \tab[2] \cmdif $\z.\bit = \w.\bit$
\State \tab[3] $\W.\CSC{\h.\Critical, \w.\seq, (\new, 1 - \w.\bit)}$ 
\State \tab[2] $\transfer{\h.\Casual}$ 

\medskip 

\Statex \tab \cmdprocedure $\transfer{\textbf{DurEC.handle} \: \h}$
\State \tab[2] $\w \gets \W.\CLL{\h.\Casual}$
\State \tab[2] \cmdfor $i \gets 1 \mbox{ to } 2$
\State \tab[3] $\z \gets \Z.\CLL{\h.\Casual}$
\State \tab[3] \cmdif $\z.\bit \neq \w.\bit$ \&\& $\W.\CVL{\h.\Casual, \w.\seq}$
\State \tab[4] \cmdif $\X.\CSC{\h.\Casual, \x.\seq, (\w.\val, \w.\bit)}$ \cmdreturn
\State \tab[2] \cmdreturn

\medskip 

\Statex \tab \cmdprocedure $\Recover{\textbf{handle*} \: \h}$
\State \tab[2] $\W.\Recover{\h.\Critical}$
\State \tab[2] $\W.\Recover{\h.\Casual}$
\State \tab[2] $\Z.\Recover{\h.\Critical}$
\State \tab[2] $\Z.\Recover{\h.\Casual}$
\State \tab[2] $\transfer{\h.\Casual}$

\medskip 

\Statex \tab \cmdstatic \cmdprocedure $\Detect{\textbf{handle*} \: \h}$
\State \tab[2] \cmdreturn $\textsc{DurEC}.\Detect{\h.\Critical}$

\end{algorithmic}
% \end{footnotesize}


\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> descriptions-old/DurEC.tex <==
\subsection{Intuitive description of Algorithm \DurEC}

Algorithm \DurEC \ implements durable EC objects from (hardware supported) atomic CAS and read operations, and it is presented in Figure~\ref{}.
Each handle $\h$ has two two persistent fields---$\h.\detval$ and $\h.\Val$, and each DurEC object $\O$ is implemented using two persistent variables $\X$ and $\Y$.
%$\X$ holds a handle $\X.\hndl$ and a sequence number $\X.\seq$, and
$\Y$ stores a sequence number $\Y.\seq$ and a value $\Y.\val$,
and the algorithm ensures that $\Y$ holds $\O$'s state at all times, i.e., $\O.\seq = \Y.\seq$ and $\O.\val = \Y.\val$ at any time.
Consequently, the $\O.\CLL{\Thandle \: \h}$ method, which by the specification must return $(\O.\seq, \O.\val)$, simply reads and returns $\Y$ (Line~4).
Similarly, the $\O.\CVL{\Thandle \: \h, \Tint \: \s}$ method, which by the specification must return the boolean $\O.\seq = s$, simply returns $\Y.\seq = \s$ (Line~5).

Next we explain the $\O.\CSC{\Thandle \: \h, \Tint \: \s, \Tint \: \v}$ method, which by the specification, returns $\false$ without changing $\O$'s state, if $\O.\seq \neq \s$; otherwise, it returns $\true$, and sets $\O.\val$ to $\v$, and $\O.\seq$ to any integer greater than $\s$.
This method's implementation uses $\X$ and the handle $\h$'s two persistent fields---$\h.\detval$ and $\h.\Val$---besides $\Y$.
At any time, $\X$ holds a handle $\X.\hndl$ and a sequence number $\X.seq$, which is either equal to or greater than $\Y.\seq$.

The algorithm is designed so that a lot of information can be inferred, based on whether $\X.\seq$ is equal to or greater than $\Y.\seq$.
Specifically, if $\X.\seq = \Y.\seq$, it simply means that there are no pending $\O.\CSC$ operations.
If $\X.\seq > \Y.\seq$, it means that there is an ongoing $\O.\CSC{\h, \s, \v}$ operation $\alpha$ about which the following inferences can be made: 
\begin{enumerate}
\item
$\alpha$'s handle $\h$ is in $\X.\hndl$ (i.e., $\X.\hndl = \h$), and we say $\h$ is {\em installed} in $\X$.
\item
$\alpha$ has already switched $\X.\seq$ from $s$ to the greater integer in $\X.\seq$, but $\Y.\seq$ still has $\s$.
\item
$\alpha$ has not linearized yet, but it is guaranteed to be the next successful $\O.\CSC$ operation to linearize.
\item
$\h.\Val$ holds $\v$, the value that $\alpha$ wants to write into $\O$ (i.e., $\X.\hndl.\Val = \v$).
% \item
% $\X.\seq \ge \h.\detval$.
\end{enumerate}

When the algorithm is in the above state, where $\X.\seq > \Y.\seq$, the handle $\h$ and any helpers are united in the mission of forwarding $\X$'s sequence number to  $\Y$, simultaneously setting $\Y.\val$ to $\v$. 
$\alpha$ linearizes at the very moment this switch happens and, since its $\CSC$ operation is successful, it will return $\true$.

In the above example, since $\alpha$ causes a change in $\Y$ (hence, a change in $\O$'s state), it is a visible operation and therefore, must be detectable.
This means that the value of $\h.\detval$ must be greater when $\alpha$ completes than when it started.
To meet this requirement, if $d$ is $\h.\detval$'s value when $\alpha$ starts, when $\alpha$ switches the sequence number in $\X$ from $\s$ to greater value $\s'$, it takes care to pick an $\s'$ that also exceeds $d$.
Once $\alpha$ changes $\X.\seq$ to $\s'$, $\h$ and any helpers ensure that $\h.\detval$ is updated from $d$ to $\s'$ before they forward the sequence number $\s'$ in $\X$ to $\Y$.
Thus, even before $\Y.\seq$ and $\Y.\val$ are updated to $\s'$ and $\v$, $\h.\detval$ increases from its earlier value of $d$ to $\s'$, thereby ensuring that $\alpha$ is detectable.

In light of the above ideas, we run through the code as a handle $\h$ executes the $\O.\CSC{\h, \s, \v}$ method.
At Line~4, if $\Y.\seq \neq \s$, it means that $\O.\seq \neq \s$; so, $\h$ returns $\false$.
Otherwise, $\h$ stores $\v$ in $\h.\Val$ to ensure that, in the event that it will be able to install itself in $\X$, helpers can know $v$ (Line~7).
Lines 8 and 9 constitute $\h$'s preparation to install itself in $\X$.
At Line~8, $\h$ notes $\X$'s current handle in $\hh$, and at Line~9, $\h$ sets $\s'$ to the sequence number it wants to store in $\X$ if it will be able to install itself in $\X$.
As explained above, it takes care to let $\s'$ be greater than both $\s$ and the current value in $\h.\detval$.
At Line~10, $\h$ executes a CAS to attempt to install itself in $\X$.
If $\h$'s CAS succeeds, its $\O.\CSC$ operation will linearize when the sequence number $\s'$ is forwarded to $\Y$ (by $\h$ or a helper).
If $\h$'s CAS fails, then some competing handle $\h'$ must have installed itself in $\X$.
In either case, $\h$ executes the helper method $\forward$ to forward the sequence number in $\X$ to $\Y$.
When $\h$ returns from forwarding and is at Line~12, it knows that whichever handle succeeded at Line~10 in installing itself in $\X$ (which may be $\h$ itself or another $\h'$), that handle's $\CSC$ operation has linearized.
If that successful handle is itself, then the response $r$ to $\h$'s CAS at Line~10 must be $\true$, which $\h$ returns.
On the other hand, if the successful handle is some $\h' \neq \h$, $\h$'s $\O.\CSC$ operation can be linearized (as a failed operation) immediately after $\h'$'s successful $\O.\CSC$ operation.
In this case, $r$ must be $\false$, which $\h$ returns.

The$\forward{\Thandle \: \h}$ \ method, if called when $\X.\seq > \Y.\seq$, accomplishes two tasks: it sets $\X.\hndl.\detval$ to $\X.\seq$ and then sets $\Y.\seq$ to $\X.\seq$, simultaneously setting $\Y.\val$ to $\X.\hndl.\Val$. The first task is accomplished by Lines 13 to 15, and the second task by Lines 13, 16, 17, and 18.

Suppose that a handle $\h$ crashes and, upon restart, executes the $\Recover$ method.
It is possible that the crash occurred while $\h$ was executing  $\O.\CSC{\h, \s, \v}$, and after $\h$ had installed itself in $\X$ and before $\X.\seq$ is moved to $\Y.\seq$, i.e., after $\h$'s $\O.\CSC{\h, \s, \v}$ operation is destined to become visible and before it linearizes.
In such a case, the call to $\forward$ \ at Line~20 forwards $\X.\seq$ to $\Y.\seq$, thereby ensuring $\h$'s visible operation linearizes before the recover method completes.

The $\Detect{\h}$ method simply returns $\h.\detval$ at Line~22.
This action fulfills the method's obligation because, as explained above, if $d$ and $d'$ are the values of $\h.\detval$ when a $\O.\CSC{\h, \s, \v}$ operation starts and completes, respectively, then $d' > d$ if the operation is visible, and $d'=d$ if the operation is not visible (and hence, is safe to repeat).

% The reading of $\X$ into $\x$ at Line~13 and the subsequent CASing of $\x.\seq$ into $\x.\hndl.\$$\X$ at Line~15 ensures that, if $\x.\hndl.\detval$ into $\sh$ (Line~14), and at Line~15, 
% Lines 14 and 15 ensure that if the installer's handle's $\detval$ (i.e., $\X.\hndl.\detval$) is less than of the installer's handle in $\X.\hndl$ into $\sh$ (Line~14). 
% The CAS at Line~15 updates the installer's handles's $\detval$ to $\sh$.
% To accomplish the second task, the installer's value $\vh$ is read from its handle's $\Val$ field (Line~16).







==> descriptions-old/DurECW.tex <==
We design Algorithm \DurECW for implementing durable objects of the ECW type (see Section~\ref{} for ECW's specification).

\subsection{Ideas underlying Algorithm \DurECW}

We describe the ideas underlying Algorithm \DurECW, which are helpful to understand before looking at the actual algorithm.

Each DurECW object $\O$ is implemented from two DurEC objects, $\W$ and $\Z$.
The crux is that $\O$'s state is held in $\Z$ at all times.
As a result, $\O.\CLL$, $\O.\CVL$, and $\O.\CSC$ are easily implemented by $\Z.\CLL$, $\Z.\CVL$, and $\Z.\CSC$.
Implementing $\O.\Write$ however, is nontrivial because of a qualitative difference between a $\O.\Write{\v}$ operation and an $\O.\CSC{\s,\v}$ operation: the write operation must plant $\v$ in $\O$ {\em unconditionally}, while the ECSC operation can simply fail (and return $\false$, making no change to $\O$'s state) if it finds the excuse that $\O$'s sequence number is not $\s$. Consequently, the algorithm must ensure that a continuous stream of successful ECSC operations do not prevent a write operation from planting its value in $\Z$.
Furthermore, the writer cannot directly plant its value $\v$ in $\Z$ since $\Z$ is a DurEC object and DurEC objects do not support the write operation. 
Thus, to ensure that a writer can unconditionally plant its value in $\Z$, in our design every ECSC operation helps any pending write before helping itself.

The DurEC object $\W$ is used, alongside $\Z$, for coordinating help between processes.
When a writer executes $\O.\Write{\v}$, it attempts to get $\v$ into $\W$ (using $\W$'s ECLL and ECSC operations).
If several write operations concurrently try to get their values into $\W$, only one of them will succeed, and we call the successful one {\em the installer}.
The failure of others is not an issue because their write operations can be linearized immediately before the point where the installer's write will be linearized.
Such linearization makes it seem that the write operations of non-installers are overwritten by the installer's write, thereby rendering non-installer's write operations invisible.
Consequently, if a non-installer crashes during its write opertation, after its subsequent restart and recovery, it can safely repeat its write operation.
In other words, the write operations by non-installers do not have to be detected.

Once writers compete to get their value into $\W$ and one of them succeeds (and becomes the ``installer''), {\em all}---the installer, the non-installer write operations, and the $\O.\CSC$ operations---make it their mission to transfer from $\W$ to $\Z$ the value just installed in $\W$.
The installer $h$ is linearized when someone successfully transfers the installed value in $\W$ to $\Z$. The non-installers, which were beaten by $h$ in the competition to install, are linearized at the same time as $h$, but are ordered before $h$.
The moment the value in $\W$ is transferred to $\Z$, $h$ ceases to be called an installer, and there is no longer a value in $\W$ to transfer to $\Z$.

To help processes determine whether $\W$ has a value to transfer, we devise an ``alternating bit protocol'', explained as follows.
As a DurEC object, $\W$'s state consists of two components---$\W.\seq$ and $\W.value$---and we use the $\W.value$ component to store a pair $(\val, \bit)$.
Thus, $\W$ can be viewed as consisting of three components, referenced as $\W = (\W.\seq, (\W.\val, \W.\bit))$.
Similarly, $\Z = (\Z.\seq, (\Z.\val, \Z.\bit))$.
We use $\W.\val$ and $\Z.\val$ for storing a value from a write or an ECSC operation, and $\W.\bit$ and $\Z.\bit$ (together with $\W.\seq$ and $\Z.\seq$) for implementing the helping scheme.
Specifically, we maintain the invariant that $\W.\bit = \Z.\bit$ if and only if there is an installer, i.e., $\W.\val$ needs to be transferred to $\Z.\val$.
More specifically, a $\Write{\v}$ operation installs by setting $\W.\val$ to $\v$ and flipping $\W.\bit$, thereby causing $\W.\bit$ and $\Z.\bit$ to be unequal.
The two bits remain unequal until some process---which can be installer, a non-installer writer, or even a process executing $\O.\CSC$---successfully transfers $\W.\val$ to $\Z.\val$ and simultaneously flips $\Z.\bit$.
When successful $\O.\CSC$ operations change $\Z$, they do not disturb $\Z.\bit$ so as not to interfere with the above alternating bit scheme to transfer installed values to $\Z$.

Next we explain the idea for achieving the detectability property.
Recall that the property states that, when a $\O.\Write$ or $\O.\CSC$ operation $\alpha$ is completed using a handle $\h$, the value of $\h.\detval$ increases if and only if $\alpha$ is visible.
To realize this property, we let a DurECW handle $h$ consist of two DurEC handles, $\h.\Casual$ and $\h.\Critical$.
When $\alpha$ performs an ECSC operation $op$ on $\W$ or $\Z$, it does so using the handle $\h.\Critical$ if $op$'s success (hence, $op$'s visibility) makes $\alpha$ a visible operation; otherwise, it uses $\h.\Casual$.
For example, when a $\O.\Write{\h, \v}$ operation $\alpha$ attempts to install $\v$ in $\W$ by performing an ECSC operation $op$ on $\W$, $\h$ becomes an installer if and only if $op$ succeeds.
Furthermore, we know that if $\h$ becomes an installer, $\alpha$ is sure to become a visible operation in the future (when its value $\v$ is transferred from $\W$ to $\Z$).
Therefore, when $\alpha$ performs $op$, it uses $\h.\Critical$ and executes $\W.\CSC{\h.\Critical, \v}$, instead of $\W.\CSC{\h.\Casual, \v}$.
On the other hand, suppose that $\alpha$ performs an ECSC operation on $\Z$, while attempting to transfer a value from $\W$ to $\Z$.
The success of this transfer (i.e., the success of the ECSC) does not affect $\alpha$'s visibility.
Therefore, in this case, $\alpha$ performs the ECSC on $\Z$ using the handle $\h.\Casual$.
Adherence to these rules ensures that, when a $\O.\Write$ or $\O.\CSC$ operation $\alpha$ is completed using a handle $\h$, the value of $\h.\Critical.\detval$ increases if and only if $\alpha$ is visible.
Thus, by defining $\h.\detval$ as $\h.\Critical.\detval$, the algorithm achieves the detectability property.

\subsection{Intuitive description of Algorithm \DurECW}

We present Algorithm \DurECW in Figure~\ref{}.
We provide here some intuition for how this algorithm implements a durable ECW object $\O$ from two durable EC objects $\W$ and $\Z$.
Our intuitive explanation is based on two key invariants that the algorithm maintains:
($I_1$) The sequence number and the value of the implemented object $\O$ are always present in $\Z.\seq$ and $\Z.\val$, and
($I_2$) $\W.\bit \neq \Z.bit$ if and only if there is an installed value in $\W.\val$ that needs to be transferred to $\Z.\val$.
We refer to these invariants repeatedly as we now turn to the code and explain how each method works.

% Turning to the code, it follows from Invariant $I_1$ that the return value of $(\z.\seq, \z.\val)$ at Line~4 is the same as $(\O.\seq, \O.\val)$. Hence, the method $\O.\CLL{\h}$ is correct.

% Consider the method $\O.\VLL{\h}$.
% At Line~5, $\Z.\VLL{\h.\Casual}$ returns $\true$ if and only if $\Z.\seq = s$.
% By Invariant $I_1$, $\Z.\seq = s$ if and only if $\O.\seq = \s$.
% Thus, the method $\O.\VLL{\h}$ returns $\true$ if and only if $\O.\seq = \s$; hence, the method is correct.

\subsubsection{The $\O.\CLL$ and $\O.\CVL$ methods}

\mbox{ }

Consider the method $\O.\CLL{\Thandle \: \h}$, which by the ECW specification must return $(\O.\seq, \O.\val)$. Since Invariant $I_1$ assures that $\O.\seq$ and $\O.\val$ are held in $\Z$, the method simply returns $(\z.\seq, \z.\val)$ at Line~4.

Consider the method $\O.\CVL{\Thandle \: \h,  \Tint \: \s}$, which by the ECW specification must return $\true$ if and only if $\O.\seq = \s$.
Since Invariant $I_1$ assures that $\O.\seq = \Z.\seq$, the method 
simply calls and returns $\Z.\CVL{\h.\Casual, \s}$ at Line~5.

\subsubsection{The $\O.\CSC$ method}

\mbox{ }

Consider the method $\O.\CSC{\Thandle \: \h,  \Tint \: \s, \Tint \: \v}$.
By the ECW specification, if $\O.\seq = \s$, this method must return $\true$, and set $\O.\val$ to $\v$, and $\O.\seq$ to a greater integer than $\s$; otherwise, it must return $\false$ without changing $\O$'s state.
At Line~6, if $\Z.\seq \neq \s$, $\O.\seq$ must also be unequal to $\s$, so the method returns $\false$.
The $\transfer{\h}$ at Line~7 helps the writers, as we will soon explain, and the relative order of Lines 7 and 8 ensures that
$\O.\CSC$ operations help the write operations before helping themselves.
At Line~8, ECSC is executed on $\Z$, which (by Invariant $I_1$) amounts to executing ECSC on $\O$.
The handle $\h.\Critical$ is used (instead of $\h.\Casual$) at this line because, if the ECSC on $\Z$ succeeds, it changes $\Z$'s state (equivalently, $\O$'s state), thereby making the method's $\O.\CSC$ operation a visible operation.
Another noteworthy point is that, even as the ECSC operation at Line~8 seeks to change $\Z.\seq$ and $\Z.\val$, it ensures that $\Z.\bit$ will remain unchanged by using the same bit $\z.\bit$ that it found in $\Z$ back at Line~6.
This care ensures that $\O.\CSC$ operations do not disturb Invariant $I_2$.

The simple check at Line~6 helps realize a useful property, which we now explain; this property will turn out to be crucial to ensuring the correctness of $\O.\Write$ operations.
Suppose that a $\O.\CSC(\h, \s, \v)$ operation by a handle $h$ does not return at Line~6.
Then, it is clear from the if-condition at Line~6 that $\h$ must have witnessed $\s$ in $\Z.\seq$.
While $\h$ is at Lines 7 or 8 and $\Z.\seq$ still has $\s$, suppose that a different handle $\h'$ performs a successful ECSC on $\Z$ at Line~8, causing $\Z.\seq$ to take on a value greater than $s$.
Then, when $\h$ subsequently executes Line~8, it is clear that $\h$'s ECSC operation on $\Z$ will fail.
We summarize this property as follows:

\begin{quote}
\underline{{\em One Shuts All} property}: Suppose that $\Z.\seq = \s$ and $S$ is a set of handles each of which witnessed $\s$ in $\Z.\seq$ and is at Lines 7 or 8. If some handle in $S$ performs a successful ECSC on $\Z$ at Line~8, then the ECSC on $\Z$ by all other handles in $S$ will fail when they perform Line~8.
\end{quote}

\subsubsection{The $\O.\Write$ method}

\mbox{ }

Next we explain the more intricate method $\O.\Write{\Thandle \: \h, \Tint \: \v}$, which by the ECW specification must set $\O.\val$ to $\v$, and $\O.\seq$ to a greater integer than what is already there.
Lines 10 to 12 constitute $\h$ attempt to get its value $\v$ installed in $\W.\val$.
The code at these lines is designed to ensure that $\h$ succeeds in making itself an installer if there is no installer  during the time interval in which $\h$ is at Line~12.
To understand how this assurance is met, suppose that there is no installer during the time interval in which $\h$ is at Line~12.
Then, $\W$ could not have changed from the time $\h$ reads $\W$ at Line~\ref{10} to the time $\h$ executes Line~12.
Furthermore, during this interval, $\W.\bit = \Z.\bit$ (by Invariant $I_2$) and, since $\O.\CSC$ operations do not change $\Z.\bit$, $\Z.\bit$ could not have changed.
Then, by the code at Lines 10 to 12, when $h$ executes Line~12, $\w.\bit = \W.\bit = \Z.\bit = \z.bit$ and $\w.\seq = \W.\seq$.
It follows that $\h$ proceeds to execute ECSC at Line~12 and the ECSC succeeds, setting $\W.\val$ to $\v$ and thereby making $\h$ the installer.
At Line~12, $\h.\Critical$ is used instead of $\h.\Casual$ because, if $h$'s $\O.\Write{\h, \v}$ method will become visible if the ECSC on $\W$ succeeds.

Regardless of whether $\h$ succeeded in becoming an installer, it calls $\transfer{\h}$ twice, at Lines 13 and 14.
The two calls together accomplish the following purpose:

\begin{quote}
\underline{{\em Two-calls} property}:
If there is an installer $I$ before $h$'s first invocation of $\transfer{\h}$, then by the time $h$ completes the second execution of $\transfer{\h}$, some handle (possibly $\h$) successfully moves the installer $I$'s value from $\W$ to $\Z$.
\end{quote}

As a result, if $\h$ had installed itself at Line~12, the value that it installed in $\W.\val$ would have moved to $\Z.\val$ by the time $\h$ completes its $\O.\Write{\h, \v}$ method; in this case, $\h$'s write operation would be linearized at the time when the installed value moved to $\Z$.
On the other hand, if $\h$ had not been successful in installing itself, let $\h^*$ be the handle that $\h$ lost out to in the installation competition.
In this case, the value that $\h^*$ installed in $\W.\val$ would have moved to $\Z.\val$ by the time $\h$ completes its $\O.\Write{\h, \v}$ method; in this case, $\h$'s write operation would be linearized immediately behind $\h^*$'s write operation, making it seem that $\h$'s write was overwritten by $\h^*$.
Thus, every $\O.\Write{\h,\v}$ operation linearizes before its completion,, whether $\h$ becomes an installer or not.

To achieve the Two-calls property, we design the $\transfer{\h}$ method to satisfy the following property:

\begin{quote}
\underline{{\em Transfer} property}:
If there is an installer at the time a handle $h$ invokes $\transfer{\h}$, then by the time $h$ completes the method, either some handle (possibly $\h$) successfully moves the installed value in $\W$ to $\Z$ or some $\O.\CSC{}$ operation performs a successful ECSC at Line~8.
 \end{quote}

We will soon explain how $\transfer{\h}$ accomplishes this property, but let us first understand how the Two-calls property follows from the Transfer and One-Shuts-All properties.
Suppose that there is an installer $I$ before $h$'s first invocation of $\transfer{\h}$ at Line~13.
If $I$'s installed value is not moved to $\Z$ by the completion of the first transfer call, the Transfer property states that some $\O.\CSC{}$ operation has performed a successful ECSC at Line~8.
Then, by One-Shuts-All property, all of the $\O.\CSC$ operations at Lines 7 or 8 will fail when they perform Line~8, so they won't be able to change $\Z$.
Any new $\O.\CSC$ operations, when they progress from Line~6 to Line~7, will call the $\transfer$ method at Line~7 before attempting to change $\Z$ at their Line~8.
Therefore, by the time $\h$ completes its second execution of $\transfer$ at Line~14, some $\transfer$ execution (not necessarily $\h$'s) would have completed without anyone executing a successful ECSC at Line~8.
Then, it follows from the Transfer property that the installed value must have moved from $\W$ to $\Z$.

\subsubsection{The $\O.\transfer$ method}

\mbox{ }

The $\transfer$ method is designed to satisfy the Transfer property stated above.
To understand how this property is achieved, suppose that,
at the time a handle $h$ invokes $\transfer{\h}$,
there is an installer, which by Invariant $I_2$ means that $\W.\bit \neq \Z.\bit$.
If during $\h$'s execution of $\transfer{\h}$ no other handle successfully moves the value in $\W$ to $\Z$ and no handle performs a successful ECSC at Line~8, then $\W$ and $\Z$ are unchanged during the time $\h$ executes Lines 16 to 18 of the transfer method.
Therefore, from an inspection of Lines 16 to 18, we see that the following statements hold at Line~18: $\zh = \Z$, $\wh = \W$, and $\W.\bit \neq \Z.\bit$. 
It follows that at Line~18, the if-condition evaluates to $\true$, causing $\h$ to execute ECSC on $\Z$, which succeeds because $\zh.\seq = \Z.\seq$. 
Thus, the value in $\W.\val$ is successfully moved to $\Z.\val$, and the Transfer property is satisfied. 

\subsubsection{The $\O.\Recover$ method}

\mbox{ }

If a handle $\h$ crashes while executing an operation on $\O$, when $\h$ subsequently restarts, it executes $\O.\Recover{\h}$.
The $\O.\Recover{\h}$ method should complete any operation on $\W$ or $\Z$ that it could be in the middle of at the time of crash, and then run its operation on $\O$ to completion.
Since $\h$ could have accessed $\W$ or $\Z$ with either of the handles $\h.\Critical$ or $\h.\Casual$, $\h$ executes Lines 19 to 22 to complete any crashed operation on $\W$ or $\Z$.
The ordering of Lines 19 to 22 is unimportant, but they must all be completed before executing Lines 23 and 24.
If $\O.\Write{\h, \v}$ crashed after becoming an installer, it would be incorrect if Lines 23 and 24 were not executed.
This is because if $\h$ became an installer and crashed before its write is successfully moved from $\W$ to $\Z$, its write might not have linearized yet; moreover, the write will become visible whenever some $\transfer$ (by any handle) will successfully move from $\W.\val$ to $\Z$.
To ensure that its write linearizes before its $\O.\Write{\h, \v}$ completes, $\h$ must execute the two calls to $\transfer$ at Lines 23 and 24.
If $\h$ is not an installer, Lines 23 and 24 are not necessary, but are harmless.









==> proofs-old/DurEC.tex <==
\section{Proof of DurEC}

We prove the DurEC algorithm using an {\em annotation-and-invariant} style proof \cite{}.
The ECLL and ECVL procedures have only a single line of code each, and are thus easy to reason about.
The principle challenge lies in reasoning about ECSC.
To address this challenge, we introduce auxiliary variables that help track the progress of each ECSC operation, and annotate some lines of the algorithm with ``annotating code'' that manipulates these variables.
The auxiliary variables and the annotation for tracking them are simply a tool to facilitate the proof of correctness. 
In particular, the annotation does not change any of the original program variables, thereby ensuring that the algorithm's behavior is unaffected by the annotation.
Nevertheless, by leveraging the auxiliary variables, we express an invariant of the algorithm that is powerful enough to imply durable linearizability and detectability of all the operations, including ECSC, thereby proving the correctness of DurEC.


% To address this challenge, we introduce auxiliary variables that help track the progress of each ECSC operation.
% Leveraging these variables, we express an invariant of the algorithm that is powerful enough to imply durable linearizability and detectability of all the operations, including ECSC, thereby proving the correctness of DurEC.

% To express how the auxiliary variables track progress, we annotate some lines of the algorithm with ``augmenting code'' that manipulate these variables.
% The auxiliary variables and the augmenting code for tracking them are simply a tool to facilitate the proof of correctness. 
% In particular, the augmenting code does not change any of the original program variables, thereby ensuring that the original algorithm's behavior is unaffected by the annotation.

\subsection{The Annotation}

We introduce the following auxiliary variables per handle $h$ to track ECSC operations:
\begin{enumerate}
    \item 
    \underline{$h.args$} stores the arguments of $h$'s ongoing ECSC operation (through crashes) when such an operation exists, and stores $\bot$ otherwise.

    % \item 
    % \underline{$h.operation$} stores the name ($h.operation.name$) and arguments ($h.operation.args$) of the handle's current operation.
    % Once the operation completes, $h.operation$ is $\bot$.
    \item
    \underline{$h.linearized$} is a boolean that stores whether $h$'s ongoing ECSC operation has linearized yet.

    \item
    \underline{$h.visible$} is a boolean that stores whether the ECSC operation had a visible effect on the object's state.

    \item
    \underline{$h.detval$} stores the value of $h.Last$ at the time that the ongoing ECSC operation was initiated if such as operation exists, and stores $\bot$ otherwise.
\end{enumerate}


The augmentations specify how the auxiliary variables are manipulated 

We express the behavior of the auxiliary tracking variables as

These auxiliary variables and the augmenting code for tracking them are simply a tool to facilitate the proof of correctness. 
In particular, the augmenting code does not change any of the original program variables, thereby ensuring that the behavior of the DurEC algorithm is unaffected.
For the augmented algorithm, we identify 

We introduce auxiliary variables 

In Figure~\ref{fig:durec-invariant} we present the invariant for the DurEC algorithm.
We adopt the following conventions in the writing of the invariant:
\begin{enumerate}
    \item 
    The full invariant $I$ is the conjunction of the invariant parts $I_1$ through $I_{10}$ displayed in the figure, quantified over all handles $h$ and all DurEC objects $\O$.

    \item
    To facilitate the expression of the invariant and its proof, we augment the algorithm with auxiliary variables and some statements that manipulate only the auxiliary variables.
    The auxiliary variables do not affect the runs of the original algorithm, and are simply a tool to prove correctness \cite{}.    
    \end{enumerate}
The augmented algorithm and invariant in figures TODO and TODO.

Our augmentation is as follows.
\begin{enumerate}
    \item 
    We introduce four auxiliary variables per handle $h$:
    \begin{enumerate}
        \item 
        \underline{$h.operation$}: stores the name ($h.operation.name$) and arguments ($h.operation.args$) of the handle's current operation.
        Once the operation completes, $h.operation$ is $\bot$.
        \item
        \underline{}
    \end{enumerate}
\end{enumerate}

Augmented variables for a handle: 
{\em operation}, {\em linearized}, {\em successful}, {\em detval}


\subimport{invariant}{DurEC}


==> proofs-old/DuraCAS-operational-proof.tex <==
\subsection{Proof of correctness of {\sc DuraCAS}}

Our first lemma confirms that, if a process crashes in the middle of an operation on $\W$ (or $\Z$), then upon restarting, the recovery method is executed on $\W$ (or $\Z$) before any other method is called on $\W$ (or $\Z$).  Consequently, $\W$ and $\Z$ exhibit a sane (i.e., durably linearizable) behavior.

\begin{lemma}\label{sanity}
{\em
Suppose that a process crashed while executing an operation $op \in \{ \mbox{\sc read}, \, \mbox{\sc write}, \mbox{\sc CAS} \}$ via a handle $\h$, and upon restarting, executes a {\sc recover}$(\h)$ operation $\alpha$.
If the process had crashed during an operation on $O \in \{\W, \Z\}$ via a handle $g \in \{ \h.\Casual, \h.\Critical \}$, the process executes $O.\mbox{\sc recover}(g)$ before executing any other operation on $O$ via handle $g$.
}
\end{lemma}

{\em Proof}: 
Suppose that $op$ is a {\sc read}$(\h)$ operation.
Then, the crash could have occurred during $\Z.\CLL{\h.\Casual}$ at Line~5, and
the lemma follows from $\alpha$'s execution of $\Z$.{\sc recover}$(\h.\Casual)$ at Line~27.

Suppose that $op$ is a {\sc write}$(\h, v)$ operation.
Then, the crash could have occurred during $\W.\CLL{\h.\Critical}$ at Line~16, or
$\Z.\CLL{\h.\Casual}$ at Line~17 or Line~23, or
$\W.\CLL{\h.\Casual}$ at Line~24, or
$\Z.\CSC{\h.\Casual}$ at Line~25.
All of these possibilities are covered by $\alpha$'s execution of the recover methods on $\W$ and $\Z$ for the handle $\h.\Casual$ at Lines 26 and 27, and the recover method on $\W$ for the handle $\h.\Critical$ at Line~30.
Furthermore, the recover methods are executed before calling at Lines 31 and 32 the {\sc transfer-write} method, which executes operations on $\W$ and $\Z$.
Hence, we have the lemma.

Suppose that $op$ is a {\sc CAS}$(\h, old, new)$ operation.
Then, the crash could have occurred during $\Z.\CLL{\h.\Critical}$ at Line~9, or
$\Z.\CLL{\h.\Casual}$ at Line~23, or
$\W.\CLL{\h.\Casual}$ at Line~24, or
$\Z.\CSC{\h.\Critical}$ at Line~13.
All of these possibilities are covered by $\alpha$'s execution of the recover methods on $\W$ and $\Z$ for the handle $\h.\Casual$ at Lines 26 and 27, and the recover method on $\Z$ for the handle $\h.\Critical$ at Line~28.
Hence, we have the lemma.
\hfill $\blacksquare$

Next we define what it means for a {\sc Write} operation to install, hitchhike, or be trivial; for a {\sc CAS} operation to imprint; and for a {\sc transfer-write} operation to move.
We will eventually prove that hitchiking writes, trivial writes, and non-imprinting CAS operations are safe to repeat; and installing writes and imprinting CAS operations are detected.

\begin{definition}
{\em 
\mbox{ }
\begin{enumerate}
\item
An {\em install} is a successful ECSC operation on $\W$, executed by a {\sc write} operation at its Line~19.

A {\sc Write} operation {\em installs a value $v$ in $\W$ at time $t$} if it executes a successful ECSC on $\W$ at Line~19 at time $t$ and sets $\W.val$ to $v$.

\item
A {\em move} is a successful ECSC operation on $\Z$, executed by a {\sc transfer-write} operation at its Line~25.

A {\sc transfer-write} operation {\em moves a value $v$ to $\Z$ at time $t$} if it executes a successful ECSC on $\Z$ at Line~25 at time $t$ and sets $\Z.val$ to $v$.

\item
An {\em imprint} is a successful ECSC operation on $\Z$, executed by a {\sc CAS} operation at its Line~13.

A {\sc CAS} operation {\em imprints a value $v$ in $\Z$ at time $t$} if it executes a successful ECSC on $\Z$ at Line~13 at time $t$ and sets $\Z.val$ to $v$.

\item
A {\sc write} operation is {\em trivial} if it completed and returned at Line~18. 

\item
A {\sc write} operation is a {\em hitchhiker} if it completed, did not install, and returned at Line~22.
\end{enumerate}
}
\hfill $\blacksquare$
\end{definition}

We adopt the following notation for referring to the time at which an operation performs an action.

\begin{definition}
{\em
If $\alpha$ is an execution of a {\sc write}, {\sc CAS}, or {\sc transfer-write} and $\ell$ is a line number in the algorithm, $\alpha[\ell]$ denotes the time at which $\alpha$ executes Line $\ell$.

Lines 9 through 13 may be executed twice because of the for-loop at Line~8,
and for any of these lines $\ell$, $\alpha[\ell,1]$ and $\alpha[\ell,2]$ denote the times at which a {\sc CAS} operation $\alpha$ executes Line $\ell$ in the first and second iterations, respectively.
}
\hfill $\blacksquare$
\end{definition}

We make two observations below about ECL objects.

\begin{observation}\label{basic}
{\em
Let $O$ be a DurEC object and $g$ and $g'$ be DurEC handles.

\begin{enumerate}
\item
If $O$.ECLL$(g)$ returns $x$ at time $t_1$, and $O$.ECSC$(g, x.seq, (v,b))$ is successful at $t_2 > t_1$, then $O$'s state remains the same (and equals $x$) in the interval $[t_1, t_2)$, and at time $t_2$, $O.val$ becomes $v$, $O.bit$ becomes $b$, and $O.seq$ becomes greater than $x.seq$.

\item
Suppose that $O$.ECLL$(g')$ returns $x'$ at time $t'_1$ and $O$.ECSC$(g', x'.seq, v')$ succeeds at a subsequent time $t'_2 > t'_1$.
Suppose also that $O$.ECLL$(g)$ returns $x$ at $t_1$, and $O$.ECSC$(g, x.seq, v)$ succeeds at $t_2 > t_1$.
If $t'_2 < t_2$, then $t'_2 < t_1$.
\end{enumerate}
}
\end{observation}

{\em Proof}: In Part (1), since the ECSC succeeds at $t_2$, $O.seq$ must be $x.seq$ at the time ECSC executes at $t_2$. 
Since $O.seq$ was $x.seq$ even at $t_1$, it follows that $O.seq$ is $x.seq$ all through the interval $[t_1, t_2)$, which implies that $O$'s state remains the same all through $[t_1, t_2)$.
Since the ECSC succeeds at $t_2$, it sets $O.val$ to $v$, $O.bit$ to $b$, and increases $O.seq$.
Hence, we have Part (1).

For a proof of Part (2), assume to the contrary that $t_1 < t'_2 < t_2$.
Since the ECSC at $t'_2$ is successful, $O.seq$ changes at time $t'_2$,
contradicting Part (1) that $O$'s state remains the same in the interval $[t_1, t_2)$.
\hfill $\blacksquare$

\begin{lemma}\label{inst1}
{\em
\mbox{ }

\begin{enumerate}
\item
If a {\sc write}$(h,v)$ operation $\alpha$ installs, then
$\W$'s state remains the same in the interval $[\alpha[16], \alpha[19])$, and
at time $\alpha[19]$, $\W.bit$ flips and $\W.val$ becomes $v$.
\item
If a {\sc transfer-write}$(h)$ operation $\alpha$ moves,
then $\Z$'s state remains the same in the interval $[\alpha[23], \alpha[25])$, and at time $\alpha[25]$, $\Z.bit$ flips.
\item
If a {\sc CAS}$(h, old, new)$ operation $\alpha$ imprints,
then $\Z$'s state remains the same in the interval $[\alpha[9,i], \alpha[13,i])$, 
where $i \in \{1,2\}$ is the iteration of the for-loop at Line~8 during which $\alpha$ imprints.
Furthermore, $old \neq new$ and, at time $\alpha[13,i]$, $\Z.val$ changes from $old$ to $new$.
\end{enumerate}
}
\end{lemma}

{\em Proof}: In Part (3), since $\alpha$ went past Lines $[10,i]$ and $[11,i]$ to execute the ECSC, we have $z.val = old \neq new$.
The rest of Part (3) and the other two parts follow from Part (1) of Observation~\ref{basic}. 
\hfill $\blacksquare$

The next lemma states that $\W$ changes only at times of installs, $\Z$ changes only at times of moves or imprints; moreover, imprints don't change $\Z.bit$.

\begin{lemma}\label{obs}
{\em
\mbox{ }
\begin{enumerate}
\item
$\W$'s state changes at time $t$ only if an install occurs at $t$.
\item
$\Z$'s state changes at time $t$ only if a move or an imprint occurs at $t$.
\item
$\Z.bit$ flips at time $t$ only if a move occurs at $t$.
\end{enumerate}
}
\end{lemma}

{\em Proof}: 
From an inspection of the algorithm, a successful ECSC on $\W$ at Line~19 is the only means to change $\W$'s state. Hence, we have Part (1) of the lemma.
Part (2) follows from the observation that a successful ECSC on $\Z$ at Line~13 or Line~25 is the only means to change $\Z$'s state.
Part (3) follows from the additional observation that Lemma~\ref{imp1} implies that a successful ECSC at Line~13 (i.e., an imprint) does not change $\Z.bit$.
\hfill $\blacksquare$

\begin{corollary}\label{cor}
{\em
\mbox{ }
\begin{enumerate}
\item
$\W.bit$ flips at time $t$ if and only if an install occurs at $t$.
\item
$\Z.bit$ flips at time $t$ if and only if a move occurs at $t$.
\end{enumerate}
}
\end{corollary}

{\em Proof}: 
The first part of the lemma follows immediately from Lemmas ~\ref{inst1} and Part (1) \ref{obs}.
The second part of the lemma follows immediately from Lemmas ~\ref{m1} and Part (1) \ref{obs}.
\hfill $\blacksquare$

\begin{lemma}\label{obs2}
{\em

\mbox{ }

\begin{enumerate}
\item
If $\alpha'$ and $\alpha$ are two different {\sc write} operations that install, and $\alpha'$ installs before $\alpha$ (i.e., $\alpha'[19] < \alpha[19]$), then $\alpha'[19] < \alpha[16]$.
\item
If $\alpha$ and $\alpha'$ are two different {\sc transfer-write} operations that move, and $\alpha'$ moves before $\alpha$ (i.e., $\alpha'[25] < \alpha[25]$), then $\alpha'[25] < \alpha[23]$.
\item
If $\alpha'$ and $\alpha$ are two different {\sc CAS} operations that imprint, and $\alpha'$ imprints at $\alpha'[13,i]$ before $\alpha$ imprints at $\alpha[13,j]$(for some $i, j \in \{1,2\}$), then $\alpha'[13,i] < \alpha[9,j]$.
\end{enumerate}
}
\end{lemma}

{\em Proof}: All three parts of the lemma are an immediate consequence of Part (2) of Observation~\ref{basic}.
\hfill $\blacksquare$

\begin{lemma}\label{ifirst}
{\em
An install occurs before any move occurs.
}
\end{lemma}

{\em Proof}: Assume to the contrary that a move occurs at time $t$ and no install occurs before $t$.
Let $\alpha$ be the {\sc transfer-write} operation that moves at $t$.
Since no installs or moves occur before $t$, Corollary~\ref{cor} implies that $\W.bit$ and $\Z.bit$ are never flipped before $t$.
So these bits still have their initial value of 0 when $\alpha$ executes ECLL at lines 23 and 24 to read the states of $\Z$ and $\W$ into $z$ and $w$, respectively.
Thus, $z.bit = w.bit$ when $\alpha$ executes Line~25.
Therefore, the if-condition at Line~25 prevents $\alpha$ from executing the ECSC operation, contradicting that $\alpha$ moves.
\hfill $\blacksquare$

The next lemma states that installs and moves alternate.

\begin{lemma}\label{rhythm}
{\em
Between any two moves, there is an install; and between any two installs, there is a move.
}
\end{lemma}

{\em Proof}: We consider two cases---that installs occur consecutively with no intervening moves or that moves occur consecutively with no intervening installs---and derive a contradiction in each case.

Suppose that the lemma is violated for the first time when an install occurs at time $t$, following an install at an earlier time $t' < t$ and with no moves in the interval from $t'$ to $t$.
Since the lemma was not violated before $t$, Corollary~\ref{cor} implies that, counting $\W$'s flip at $t'$, $\W$ is flipped one more time than $\Z$ by time $t'$, and no further flips happen to either bit in the open interval from $t'$ to $t$.
It follows that, in the open interval from $t'$ to $t$, the values of $\W.bit$ and $\Z.bit$ do not change and, since $\W.bit$ and $\Z.bit$ are both initially 0, $\W.bit \neq \Z.bit$.
Let $b$ and $1-b$ be the stable values of $\W.bit$ and $\Z.bit$, respectively, in the interval $(t',t)$.
Let $\alpha'$ and $\alpha$ denote the {\sc write} operations that install at times $t'$ and $t$, respectively; thus, $t' = \alpha'[19]$ and $t = \alpha[19]$.
From Part (1) of Lemma~\ref{obs2}, we know that $\alpha'[19] < \alpha[16] < \alpha[19]$.
Then, since $\W.bit$ and $\Z.bit$ remain unchanged at $b$ and $1-b$ from $\alpha'[19]$ to $\alpha[19]$, when $\alpha$ executes ECLL at Lines 16 and 17 to read $\W$'s state and $\Z$'s state into $w$ and $z$, respectively, $w.bit$ is set to $b$ and $z.bit$ is set to $1-b$.
Therefore, when $\alpha$ executes Line~19, the if-condition there evaluates to {\em false}, preventing $\alpha$ from executing the ECSC operation, which contradicts that $\alpha$ installs.

The second case is argued analogously.
Suppose that the lemma is violated for the first time when a move occurs at time $t$, following a move at an earlier time $t' < t$ and with no installs in the interval from $t'$ to $t$.
Since the lemma was not violated before $t$, Corollary~\ref{cor} implies that, counting $\Z$'s flip at $t'$, $\W$ and $\Z$ are flipped the same number of times by time $t'$, and no further flips happen to either bit in the open interval from $t'$ to $t$.
It follows that, in the open interval from $t'$ to $t$, the values of $\W.bit$ and $\Z.bit$ do not change and, since $\W.bit$ and $\Z.bit$ are both initially 0, $\W.bit = \Z.bit$.
Let $b$ be the stable value of $\W.bit$ in the interval $(t',t)$.
Let $\alpha'$ and $\alpha$ denote the {\sc transfer-write} operations that move at times $t'$ and $t$, respectively; thus, $t' = \alpha'[25]$ and $t = \alpha[25]$.
From Part (2) of Lemma~\ref{obs2}, we know that $\alpha'[25] < \alpha[23] < \alpha[25]$.
Then, since $\W.bit$ and $\Z.bit$ remain unchanged at $b$ from $\alpha'[19]$ to $\alpha[19]$, when $\alpha$ executes ECLL at Lines 23 and 24 to read $\Z$'s state and $\W$'s state into $z$ and $w$, respectively, both $w.bit$ and $z.bit$ are set to $b$.
Therefore, when $\alpha$ executes Line~25, the if-condition there evaluates to {\em false}, preventing $\alpha$ from executing the ECSC operation, which contradicts that $\alpha$ moves.
\hfill $\blacksquare$

\begin{corollary}\label{seesaw}
{\em
\mbox{ }

\begin{enumerate}
\item
$\W.bit$ and $\Z.bit$ do not change and have the same value in the open interval up to the first install and in each open interval from a move to the first install that follows that move.
\item
$\W.bit$ and $\Z.bit$ do not change and have different values in each open interval from an install to the move that first follows that install.
\end{enumerate}
}
\end{corollary}

{\em Proof}: The two parts of the lemma follow immediately from Lemma~\ref{rhythm}, Corollary~\ref{cor}, and the fact that both $\W.bit$ and $\Z.bit$ are initially 0.
\hfill $\blacksquare$

\begin{lemma}\label{snap}
{\em
\mbox{ }

\begin{enumerate}
\item
If a {\sc write} operation $\alpha$ installs, then $\W.bit = \Z.bit$ at time $\alpha[17]$.
\item
If a {\sc transfer-write} operation $\alpha$ moves, then $\W.bit \neq \Z.bit$ at time $\alpha[24]$.
\end{enumerate}
}
\end{lemma}

{\em Proof}:
Since $\alpha$ is successful, it follows from Lemma~\ref{inst1} that $\W$'s state does not change in the open interval from $\alpha[16]$ to $\alpha[19]$.
Therefore, $w$, which is $\W$'s state returned by $\alpha$'s ECLL at Line~16, continues to be $\W$'s state at $\alpha[19]$.
The ECLL on $\Z$ at Line~17 returns $\Z$'s state at $\alpha[17]$ into $z$.
Thus, the values of $\W.bit$ and $\Z.bit$ at time $\alpha[17]$ are $w.bit$ and $z.bit$, respectively.
Since $\alpha$ installs (i.e., executes a successful ECSC at Line~19), the if-condition at Line~19 must evaluate to {\em true}, which implies that $z.bit = w.bit$, which from the above implies that $\W.bit = \Z.bit$ at time $\alpha[17]$.
Hence, we have Part (1) of the lemma.

Part (2) is proved analogously.
Since $\alpha$ is successful, it follows from Lemma~\ref{m1} that $\Z$'s state does not change in the open interval from $\alpha[23]$ to $\alpha[25]$.
Therefore, $z$, which is $\Z$'s state returned by $\alpha$'s ECLL at Line~23, continues to be $\Z$'s state at $\alpha[24]$.
The ECLL on $\W$ at Line~24 returns $\W$'s state at $\alpha[24]$ into $w$.
Thus, the values of $\W.bit$ and $\Z.bit$ at time $\alpha[24]$ are $w.bit$ and $z.bit$, respectively.
Since $\alpha$ moves (i.e., executes a successful ECSC at Line~25), the if-condition at Line~25 must evaluate to {\em true}, which implies that $z.bit \neq w.bit$, which from the above implies that $\W.bit \neq \Z.bit$ at time $\alpha[24]$.
\hfill $\blacksquare$

\begin{lemma}\label{wtozhelp}
{\em
\mbox{ }

\begin{enumerate}
\item
If an install occurs at time $t$ and the first move after $t$ is executed by a {\sc transfer-write} operation $\alpha$, then $\alpha[24] > t$.
\item
If a move occurs at time $t$, and the first install after $t$ is executed by a {\sc write} operation $\alpha$, then $\alpha[17] > t$.
\end{enumerate}
}
\end{lemma}

{\em Proof}: For a proof of Part (1), assume for a contradiction that $\alpha[24] < t$.
Part (2) of Lemma~\ref{snap} implies that $\W.bit \neq \Z.bit$ at time $\alpha[24]$.
Therefore, the instant $\alpha[24]$ falls in a time interval where $\W.bit \neq \Z.bit$.
If the install at $t$ is not the first install, let $t'$ be the latest time before $t$ when a move occurs.
Corollary~\ref{seesaw} implies that $\W.bit = \Z.bit$ during the open interval from $t'$ to $t$, and $\W.bit \neq \Z.bit$ during the open interval from $t$ to $\alpha[25]$.
Then, since $\alpha[24] < t$ and $\alpha[24]$ falls in a time interval where $\W.bit \neq \Z.bit$,
it must be that $\alpha[24] < t'$.
Since $\alpha$ moves after $t$, $\alpha[25] > t$.
It follows from the above that $\alpha[24] < t' < t < \alpha[25]$.
Since a move occurs at $t'$, there is a successful ECSC on $\Z$ at $t'$.
Therefore, $\Z$'s state changes at $t'$, which implies that
$\Z$'s state changes between $\alpha[24]$ and $\alpha[25]$, contradicting Lemma~\ref{m1} that states that $\Z$'s state does not change in the interval from $\alpha[23]$ to $\alpha[25]$.
Hence, we have Part (1) of the lemma.

For an analogous proof of Part (2), assume for a contradiction that $\alpha[17] < t$.
Part (1) of Lemma~\ref{snap} implies that $\W.bit = \Z.bit$ at time $\alpha[17]$.
Therefore, the instant $\alpha[17]$ falls in a time interval where $\W.bit = \Z.bit$.
Let $t'$ be the latest time before $t$ when an install occurs.
Corollary~\ref{seesaw} implies that $\W.bit \neq \Z.bit$ during the open interval from $t'$ to $t$, and $\W.bit = \Z.bit$ during the open interval from $t$ to $\alpha[19]$.
Then, since $\alpha[17] < t$ and $\alpha[17]$ falls in a time interval where $\W.bit = \Z.bit$,
it must be that $\alpha[17] < t'$.
Since $\alpha$ installs after $t$, $\alpha[19] > t$.
It follows from the above that $\alpha[17] < t' < t < \alpha[19]$.
Since an install occurs at $t'$, there is a successful ECSC on $\W$ at $t'$.
Therefore, $\W$'s state changes at $t'$, which implies that
$\W$'s state changes between $\alpha[17]$ and $\alpha[19]$, contradicting Lemma~\ref{inst1} that states that $\W$'s state does not change in the interval from $\alpha[16]$ to $\alpha[19]$.
Hence, we have Part (2) of the lemma.
\hfill $\blacksquare$

The next lemma states that if two {\sc transfer-write} operations are executed after installing a value $v$ in $\W$, $v$ is sure to move to $\Z$ by the end of the second transfer-write operation.

\begin{lemma}\label{tran}
{\em
If $\W.bit \neq \Z.bit$ at time $t$,
a {\sc transfer-write} operation $\alpha_1$ is started after $t$, and another {\sc transfer-write} operation $\alpha_2$ is started after $\alpha_1$ completes, then a move occurs  after $t$ and at or before $\alpha_2$'s completion time of $\alpha_2[25]$.
}
\end{lemma}

{\em Proof}: Assume to the contrary that no move occurs between $t$ and $\alpha_2[25]$.
Then, Corollary~\ref{seesaw} implies that, in the interval from $t$ to $\alpha_2[25]$, $\W.bit$ and $\Z.bit$ do not change and $\W.bit \neq \Z.bit$.
Let $b \in \{0,1\}$ and $1-b$ be $\W.bit$'s value and $\Z.bit$'s value, respectively, in this interval.
Therefore, in both $\alpha_1$ and $\alpha_2$, the ECLL operations on $\Z$ and $\W$ at Lines 23 and 24 return $z$ and $w$ such that $z.bit = 1-b$ and $w.bit = b$;
so, the if-condition at Line~25 evaluates to {\em true} and the ECSC operation on $\Z$ is attempted.
However, by our assumption that no move occurs by time $\alpha_2[25]$, the ECSC on $\Z$ at Line~25 is unsuccessful in both $\alpha_1$ and $\alpha_2$.

The failure of $\alpha_1$'s ECSC at Line~25 must be because $\Z$'s state changed between $\alpha_1$'s ECLL at Line~23 and its subsequent ECSC at Line~25.
Therefore, by Lemma~\ref{obs}, an imprint or a move occurs between $\alpha_1[23]$ and $\alpha_1[25]$.
It must be an imprint because a move is ruled out by our assumption that no move occurs by time $\alpha_2[25]$.
Let $\beta_1$ be the {\sc CAS} operation that imprints between $\alpha_1[23]$ and $\alpha_1[25]$.
Arguing similarly, there is a {\sc CAS} operation $\beta_2$ that imprints between $\alpha_2[23]$ and $\alpha_2[25]$.
Let $i_1 \in \{1,2\}$ and $i_2 \in \{1,2\}$ be the iterations (of the for-loop at Line~8) during which $\beta_1$ and $\beta_2$, respectively, execute a successful ECSC on $\Z$.
Lemma~\ref{imp1} implies that $\Z$'s state is unchanged in the open interval from $\beta_2[9,i_2]$ and $\beta_2[13,i_2]$.

Since $\beta_1$ imprints between $\alpha_1[23]$ and $\alpha_1[25]$, we have $\alpha_1[23] < \beta_1[13,i_1] < \alpha_1[25]$.
Similarly, we have $\alpha_2[23] < \beta_2[13,i_1] < \alpha_2[25]$.
Furthermore, Part (3) of Lemma~\ref{obs2} implies that $\beta_1[13,i_1] < \beta_2[9,i_2]$.
Putting these together, we have $t < \alpha_1[23] < \beta_1[13,i_1] < \beta_2[9,i_2] < \beta_2[13,i_2] < \alpha_2[25]$.
In particular, $t < \beta_2[9,i_2] < \beta_2[13,i_2] < \alpha_2[25]$.
Furthermore, Lemma~\ref{imp1} implies that $\Z$'s state is unchanged in the open interval from $\beta_2[9,i_2]$ and $\beta_2[13,i_2]$; in particular, $\Z$'s state is constant throughout the time that $\beta_2$ calls and executes {\sc transfer-write} from Line$[12,i_2]$.
The last two observations imply that, during this execution of {\sc transfer-write},
$\beta_2$'s ECLL on $\Z$ at Line~23 returns a $z$ such that $z.bit = 1-b$, its ECLL on $\W$ at Line~24 returns a $w$ such that $w.bit = b$, and $\Z$'s state is still $z$ when $\beta_2$ executes Line~25.
It follows that the if-condition at Line~25 evaluates to {\em true}, so $\beta_2$ executes the ECSC operation; and this ECSC succeeds because $\Z$'s state is unchanged between Lines~23 and 25.
This successful ECSC means that $\beta_2$ moves, contradicting our assumption that no move occurs between $t$ and $\alpha_2[25]$.
\hfill $\blacksquare$

The next lemma states that if a {\sc write} operation $\alpha$ installs a value $v$ in $\W$, that value is moved to $\Z$ before $\alpha$ completes.

\begin{lemma}\label{wok}
{\em
If a {\sc write}$(h,v)$ operation $\alpha$ installs $v$ at time $t$, the first move after $t$ occurs before $\alpha$ completes and it moves $v$ to $\Z$.
}
\end{lemma}

{\em Proof}: After $\alpha$ installs at time $t$ (by executing a successful ECSC on $\W$ at Line~19), $\alpha$ executes the {\sc transfer-write} method twice (at Lines 20 and 21) before completing.
If the process $p$ executing $\alpha$ crashes before executing {\sc transfer-write} twice, upon restart, $p$ executes the {\sc recover} method where, after recovering from any partially executed operations on $\W$ and $\Z$ (invoked via either handle) at Lines 26, 27, and 30, {\sc transfer-write} is executed twice, at Lines 31 and 32.
Thus, after $\alpha$ installs at time $t$, regardless of crashes, $\alpha$ executes {\sc transfer-write} at least twice, before completing.
It follows from Lemma~\ref{tran} that a move occurs before $\alpha$ is completed.
Hence, we have the first part of the lemma.

Let $\alpha'$ be the {\sc transfer-write} operation that executes the first move after $t$.
$\W.val$ becomes $v$ at time $t$ (by Lemma~\ref{inst1}) and continues to be $v$ until $\alpha'$ moves, i.e., until $\alpha'[25]$ (by Lemma~\ref{obs}).
Furthermore, $\alpha'[24] > t$ (by Lemma~\ref{wtozhelp}).
It follows from the above that, when $\alpha'$ reads $\W$ into $w$ at Line~24, $w.val = v$.
Therefore, when $\alpha'$ moves by executing a successful ECSC on $\Z$ at Line~25, the passing of $w.val$ as the third argument of that $ECSC$ ensures that $\Z.val$ is set to $v$.
This concludes the proof that the first move after $t$ moves $v$ to $\Z$.
\hfill $\blacksquare$

The next lemma states that if a value $v$ is moved to $\Z$ and there are no imprints after the move, then the next installed value can't be $v$.
This property is crucial to ensuring the correctness and wait-freedom of CAS operations in the face of an unbounded stream of write operations that write the same value.

\begin{lemma}\label{norepeat}
{\em
If a move occurs at time $t'$, an install occurs at time $t > t'$, and no imprints occur between $t'$ and $t$, then the value installed at $t$ differs from the value moved at $t'$.
}
\end{lemma}

{\em Proof}: Let $v'$ be the value moved at $t'$ and $\alpha$ be the {\sc write}$(h,v)$ operation that installs at $t$.
Assume that no imprints occur between $t'$ and $t$. 
We need to prove that $v \neq v'$.
The move at $t'$ sets $\Z.val$ to $v'$, and
since no moves or imprints occur in the open interval from $t'$ to $t = \alpha[19]$, 
$\Z.val$ remains at $v'$ throughout this interval.
Furthermore, $\alpha[17] > t$ (by Part (2) of Lemma~\ref{wtozhelp}).
Therefore, $\alpha$'s ECLL on $\Z$ at Line~17 returns $z$ such that $z.val = v'$.
Therefore, if $v'$ were the same as $v$, the if-condition at Line~18 would cause $\alpha$ to return at Line~18, contradicting that $\alpha$ installs.
We conclude that $v' \neq v$.
\hfill $\blacksquare$

Recall that a hitchhiker is a {\sc write} operation that does not install and returns at Line~22.

\begin{lemma}\label{hh1}
{\em
If $\alpha$ is a hitchhiker {\sc write} operation, $\W.bit \neq \Z.bit$ at some time between $\alpha[16]$ and $\alpha[19]$.
}
\end{lemma}

{\em Proof}: Assume $\W.bit = \Z.bit$ all through the interval from $\alpha[16]$ to $\alpha[19]$.
Then, Corollary~\ref{seesaw} implies that in this interval $\W$'s state and $\Z.bit$ do not change their values.
It follows that, when $\alpha$ executes an ECLL on $\W$ and $\Z$ at Lines 16 and 17, the return values $w$ and $z$ are such that $w.bit = z.bit$ and $W$'s state continues to be $w$ at $\alpha$'s Line~19.
Since $\alpha$ is a hitchhiker, it does not return at Line~18, the if-condition at Line~19 evaluates to {\em true}, and the ECSC at Line~19 succeeds (since $\W.seq$ equals ECSC's second argument $w.seq$).
Thus, $\alpha$ installs, contradicting that $\alpha$ is a hitchhiker.
\hfill $\blacksquare$

The next lemma states that a move occurs during every hitchhiking write.

\begin{lemma}\label{hh}
{\em
If $\alpha$ is a hitchhiker {\sc write} operation, a move occurs between $\alpha[16]$ and $\alpha[22]$.
}
\end{lemma}

{\em Proof}: By the previous lemma, $\W.bit \neq \Z.bit$ at some time $t$ between $\alpha[16]$ and $\alpha[19]$. Since $\alpha$ executes two {\sc transfer-write} operations after $\alpha[16]$ and before it returns at Line~22, Lemma~\ref{tran} implies that a move occurs between $t$ and $\alpha[22]$.
Hence, we have the lemma.
\hfill $\blacksquare$

The next definition states which {\sc write} operations are linearized and where.

\begin{definition}\label{wlin}
{\em
Let $\alpha$ be a {\sc write}$(h,v)$ operation.

\begin{enumerate}
\item
If $\alpha$ installs, it is linearized at the time $t$ of the first move after $\alpha$ installs.
(Lemma~\ref{wok} guarantees that $t$ lies within the interval of $\alpha$'s execution.)
\item
If $\alpha$ is a hitchhiker, it is linearized at the time $t$ of the first move that occurs within the interval of $\alpha$'s execution. (Lemma~\ref{hh} guarantees the existence of $t$.)
\item
If $\alpha$ is trivial (i.e., returns at Line~18), it is linearized at $\alpha[17]$, the time where $\alpha$ executes Line~17.
\end{enumerate}
}
\hfill $\blacksquare$
\end{definition}

\begin{observation}\label{obs3}
{\em
Exactly one installing {\sc write} operation is linearized at each move.
}
\end{observation}

{\em Proof}: Let $t$ be the time of any move.
Since installs and movers alternate (Lemma~\ref{rhythm}), there is a unique install $i$ such that the first move after $i$ occurs at $t$. Then, by our definition of Linearizability, the {\sc write} operation whose install is $i$ is the unique installing {\sc write} operation that is initialized at time $t$.
\hfill $\blacksquare$

Even though our definition ensures only one installing write is linearized at the time of a move, any number (possibly zero) of hitchhiker writers may linearize at the same time.
The rule below states how to order multiple {\sc write} operations that all linearize at the same time.

\begin{definition}\label{wlin2}
{\em
If a move occurs at time $t$, and a nonempty set $S$ of hitchhiker {\sc write} operations along with a unique installing {\sc write} operation $\alpha$ are linearized at $t$, in the linearization order the {\sc write} operations in $S$ are placed (in an arbitrary total order) {\em behind} $\alpha$.
(Intuitively, they all ``take effect'' at $t$, but the writes in $S$ are overwritten by $\alpha$.)
}
\end{definition}

The next definition states which {\sc CAS} operations are linearized and where.

\begin{definition}\label{clin}
{\em
Let $\alpha$ be a {\sc CAS}$(h, old, new)$ operation.

\begin{enumerate}
\item
If $\alpha$ imprints, it is linearized at the time it imprints.
\item
If $\alpha$ completes by returning at Line~$[10,i]$ or at Line~$[11,i]$, for $i \in \{1,2\}$, it is linearized at $\alpha[9,i]$.
\end{enumerate}
}
\hfill $\blacksquare$
\end{definition}

\begin{definition}\label{rlin}
{\em 
If a {\sc read} operation $\alpha$ completes, it is linearized at $\alpha[5]$.
}
\hfill $\blacksquare$
\end{definition}


\begin{lemma}\label{lin}
{\em 
\mbox{ }
\begin{enumerate}
\item
If an operation completes without crashing, it is linearized.
\item
If an operation is linearized, the time at which it is linearized falls in the interval of that operation.
\end{enumerate}
}
\end{lemma}

{\em Proof}: A {\sc write} that completes without crashing is trivial, or installs, or a hitchhiker, and is linearized in all cases (by Definition~\ref{wlin}).
A {\sc CAS} that completes without crashing imprints, or returns at Line~$[10,i]$ or $[11,i]$ (for some $i \in \{1,2\})$, and is linearized in all cases (by Definition~\ref{clin}).
A {\sc read} that completes without crashing returns at Line~6, and is linearized (by Definition~\ref{rlin}).
Hence, we have Part (1) of the lemma.

It is obvious from Definitions \ref{wlin}, \ref{clin}, and \ref{rlin} that if an operation linearizes, its linearization time falls within the interval of the operation. Hence, we have Part (2).
\hfill $\blacksquare$

The next lemma states that the value of the implemented DuraCAS object $\mathcal O$ is always present in $\Z.val$, and that every linearized ({\sc read}, {\sc CAS}, or {\sc write}) operation correctly changes $\mathcal O$'s value and, if the operation completes without crashing, returns a correct response. (When a crashed operation is completed via the {\sc recover} method, no response is returned even if the operation is linearized.)

\begin{lemma}\label{juice}
{\em 
Let $\mathcal O$ denote the DuraCAS object implemented by the algorithm, and ${\mathcal O}.val$ denote $\mathcal O$'s value.

\begin{enumerate}
\item
${\mathcal O}.val = \Z.val$ at all times.
\item
If one or more operations on $\mathcal O$ are linearized at time $t$, these operations correctly change ${\mathcal O}.val$ at $t$, i.e., they change ${\mathcal O}.val$ consistent with the sequential specification.
\item
If an operation on $\mathcal O$ completes without crashing, it returns a correct response, i.e., a response consistent with the sequential specification.
\item
Hitchhiker {\sc write} operations, trivial {\sc write} operations, {\sc CAS} operations that return at Line~10 or at Line~11, and {\sc read} operations are safe to repeat.
\end{enumerate}
}
\end{lemma}

{\em Proof}: We note that ${\mathcal O}.val$ and $\Z.val$ change only at discrete times: ${\mathcal O}.val$ changes only at linearization times and $\Z.val$ changes only at times of moves and imprints, which are linearization times. So, we prove the lemma by by induction as follows.

The base step follows from the algorithm's initialization that sets $\Z.val$ to $\mathcal O$'s initial value.
For the induction hypothesis, assume that $i \ge 1$ and the lemma holds up to and including the first $i-1$ linearization times.
Let $\tau$ be the next linearization time and $S$ be the set of operations that are linearized at $\tau$.
For the induction step, we show that the lemma holds even after the operations in $S$ take effect at $\tau$ (in their linearization order).
There are many possibilities for what operations are linearized at $\tau$, and we show the induction step below for each possibility.

\begin{itemize}
\item
\underline{Case 1, move occurs at $\tau$}:
In this case, a set $S$ of hitchhiker {\sc write} operations and one installing {\sc write}$(h,v)$ operation $\alpha$ are linearized, all at $\tau$, but with $\alpha$ linearizing after the ones in $S$ (Observation~\ref{obs3} and Definition~\ref{wlin2}). As a result, all hitchhiker writes are overwritten by $\alpha$, and ${\mathcal O}.val$ becomes $v$ at time $\tau$. Since the hitchhiker writes are overwritten, they are safe to repeat. The hitchhiker writes in $S$ return {\em ack} at Line~22 and, if $\alpha$ completes without crashing, it also returns {\em ack} at Line~22. Furthermore, the move at $\tau$ sets $\Z.val$ to $v$ at $\tau$ (Lemma~\ref{wok}), thereby ensuring that ${\mathcal O}.val = \Z.val$ immediately after $\tau$.

\underline{Case 2, imprint occurs at $\tau$}:
In this case, the {\sc CAS}$(h, old, new)$ operation $\alpha$ that imprints at $\tau$ is linearized at $\tau$.
Then, $\Z.val$ changes from $old$ to $new$ at $\tau$ (Lemma~\ref{imp1}).
By the induction hypothesis, immediately before $\alpha$'s linearization at $\tau$, ${\mathcal O}.val = \Z.val = old$, and $\alpha$'s linearization changes ${\mathcal O}.val$ from $old$ to $new$.
Furthermore, if $\alpha$ does not crash after imprinting (i.e., after the successful ECSC at Line~13), it returns the correct response of {\em true} at Line~13.

\underline{Case 3, a trivial write is linearized at $\tau$}:
In this case, a {\sc write}$(h,v)$ operation $\alpha$, which reads $v$ in $\Z.val$  at Line~17 at time $\tau$ and returns at the next line, is linearized at $\tau$.
Thus, immediately before $\alpha$'s linearization at $\tau$, $\Z.val = v$ and, by the induction hypothesis, ${\mathcal O}.val = v$. 
Immediately after $\alpha$'s linearization at $\tau$, $\Z.val$ continues to be $v$ (because $\Z$ is not changed at $\tau$ by $\alpha$'s implementation code) and ${\mathcal O}.val$ also continues to be $v$ because $\alpha$'s {\sc write}$(h,v)$ operation takes effect at $\tau$, changing ${\mathcal O}.val$ from $v$ to $v$.
Thus, the trivial write $\alpha$ does not change ${\mathcal O}.val$, so it is safe to repeat.

\underline{Case 4, a {\sc CAS}$(h,old,new)$ operation $\alpha$, which returns at Line~10, is linearized at $\tau$}:
In this case, since CAS operations returning at Line~10 are linearized at the time they execute the previous line, $\tau$ is the time of $\alpha$'s execution of Line~9.
It follows from the code at Lines 9 and 10 that $\Z.val \neq old$ when $\alpha$ executes Line~9 at $\tau$.
By the induction hypothesis, ${\mathcal O}.val \neq old$ at $\tau$, so $\alpha$'s linearization at $\tau$ implies that ${\mathcal O}.val$ remains unchanged, and ${\mathcal O}$'s response is {\em false}. This justifies $\alpha$ returning {\em false} at Line~10, without changing $\Z$. 
Finally, since $\alpha$ returns {\em false}, it is safe to repeat.

\underline{Case 5, a {\sc CAS}$(h,old,new)$ operation $\alpha$, which returns at Line~11, is linearized at $\tau$}:
In this case, since CAS operations returning at Line~11 are linearized at the time they execute Line~9, $\tau$ is the time of $\alpha$'s execution of Line~9.
In this case, it follows from the code at Lines 9, 10, and 11 that $old$ and $new$ are the same value $v$ and $\Z.val = v$ when $\alpha$ executes Line~9 at $\tau$.
By the induction hypothesis, ${\mathcal O}.val = v$ at $\tau$, so $\alpha$'s linearization at $\tau$ implies that ${\mathcal O}.val$ changes from $v$ to $v$ (i.e., ${\mathcal O}.val$) is unchanged, and ${\mathcal O}$'s response is {\em true}. 
This justifies $\alpha$ returning {\em true} at Line~11, without changing $\Z$. 
Finally, even though ${\mathcal O}$'s response to $\alpha$ is {\em true}, since $\alpha$ does not change ${\mathcal O}.val$, it is safe to repeat.

\underline{Case 6, a {\sc read}$(h)$ operation $\alpha$ is linearized at $\tau$}:
In this case, $\tau$ is the time of $\alpha$'s execution of Line~5.
Since $\O.val = \Z.val$ at $\tau$ (by the induction hypothesis), $\alpha$'s linearization at $\tau$ implies that ${\mathcal O}.val$ remains unchanged, and ${\mathcal O}$'s response is $\Z.val$ at $\tau$, which is $z.val$.
This justifies $\alpha$ returning $z.val$ at Line~11, without changing $\Z$.
Finally, since $\alpha$ is a {\sc read} and does not change ${\mathcal O}$'s state, it is safe to repeat.
\end{itemize}

Hence, the induction step is complete and we have the lemma.
\hfill $\blacksquare$

Next we prove the properties of DuraCAS objects that make them detectable. 

\begin{lemma}\label{det}
{\em 
\mbox{ }
\begin{enumerate}
\item
All operations except installing {\sc write} operations and imprinting {\sc CAS} operations are safe to repeat.
\item
If {\sc detect}$(h)$ is executed before and after a {\sc write}$(h,v)$ operation $\alpha$ that installs, and the first and the second execution of {\sc detect} return $(d_1, r_1)$ and $(d_2,r_2)$ respectively, then $d_2 > d_1$ and $r_2 = \mbox{\em true}$.
\item
If {\sc detect}$(h)$ is executed before and after a {\sc CAS}$(h,old, new)$ operation $\alpha$ that imprints, and the first and the second execution of {\sc detect} return $(d_1, r_1)$ and $(d_2,r_2)$ respectively, then $d_2 > d_1$ and $r_2 = \mbox{\em ack}$.
\item
If {\sc detect}$(h)$ is executed before and after any operation $\alpha$ that is not an installing write or imprinting CAS, and the first and the second execution of {\sc detect} return $(d_1, r_1)$ and $(d_2,r_2)$ respectively, then $d_2 = d_1$.
\end{enumerate}
}
\end{lemma}

{\em Proof}:
Part (1) of the lemma follows from Part (4) of Lemma~\ref{juice}.

In Part (2), since $\alpha$ installs, its ECSC on $\W$, performed at Line~19, using the handle $\h.\Critical$, is successful.
Besides this successful ECSC, $\alpha$ does not attempt any ECSC (on $\W$ or $\Z$) using the handle $\h.\Critical$.
Therefore, the detectability of DurEC objects implies that, when the two successive executions of {\sc detect} obtain $d_1$ and $d_2$ at their Line~33, we have $d_2 > d_1$. Furthermore, since $\h.op = \mbox{Write}$ when {\sc Detect} is called the second time, the second {\sc Detect} returns $(d_2, ack)$ at Line~34. Hence, we have Part (2) of the lemma.

Proof of Part (3) is similar.
Since $\alpha$ imprints, its ECSC on $\Z$, performed at Line~$[13,i]$, using the handle $\h.\Critical$, is successful.
Besides this successful ECSC, $\alpha$ does not attempt any ECSC (on $\W$ or $\Z$) using the handle $\h.\Critical$.
Therefore, the detectability of DurEC objects implies that, when the two successive executions of {\sc detect} obtain $d_1$ and $d_2$ at their Line~33, we have $d_2 > d_1$. Furthermore, since $\h.op = \mbox{CAS}$ when {\sc Detect} is called the second time, the second {\sc Detect} returns $(d_2, true)$ at Line~34. Hence, we have Part (3) of the lemma.

In Part (4), since $\alpha$ neither installs nor imprints, it does not perform any successful ECSC on $\W$ or $\Z$.
Therefore, the detectability of DurEC objects implies that, when the two successive executions of {\sc detect} obtain $d_1$ and $d_2$ at their Line~33, we have $d_2 = d_1$.
Hence, we have Part (4) of the lemma.
\hfill $\blacksquare$

\begin{theorem}\label{durlin}
{\em 
DuraCAS objects are durably linearizable and detectable.
All operations are wait-free and run in constant time.
The space complexity is fully adaptive and linear: $O(m+n)$ space is used in a run where $m$ DuraCAS objects are created and $n$ processes participate (by calling {\sc CreateHandle} to acquire a handle).
}
\end{theorem}

{\em Proof}: Durable linearizability of DuraCAS objects follows immediately from Lemma~\ref{lin} and Parts (2) and (3) of Lemma~\ref{juice}.
The detectability of DuraCAS objects follows immediately from Lemma~\ref{det}.
That all operations are wait-free and run in constant time is obvious from inspecting the algorithm.
Each DuraCAS handle needs space for two DurEC handles and for a field to store an operation, so needs constant space.
Each DuraCAS object has two instance variable, which are the DurEC objects $\W$ and $\Z$, so a DuraCAS object needs constant space.
Therefore, if $m$ DuraCAS objects are created and $n$ processes choose to share them, the total space used is $O(m+n)$.
\hfill $\blacksquare$





==> proofs-old/invariant/DurEC.tex <==
\section{Proof of DurEC}

We prove the DurEC algorithm using an {\em annotation-and-invariant} style proof \cite{}.
The ECLL and ECVL procedures have only a single line of code each, and are thus easy to reason about.
The principle challenge lies in reasoning about ECSC.
To address this challenge, we introduce auxiliary variables that help track the progress of each ECSC operation, and annotate some lines of the algorithm with ``annotating code'' that manipulates these variables.
The auxiliary variables and the annotation for tracking them are simply a tool to facilitate the proof of correctness. 
In particular, the annotation does not change any of the original program variables, thereby ensuring that the algorithm's behavior is unaffected by the annotation.
Nevertheless, by leveraging the auxiliary variables, we express an invariant of the algorithm that is powerful enough to imply durable linearizability and detectability of all the operations, including ECSC, thereby proving the correctness of DurEC.


% To address this challenge, we introduce auxiliary variables that help track the progress of each ECSC operation.
% Leveraging these variables, we express an invariant of the algorithm that is powerful enough to imply durable linearizability and detectability of all the operations, including ECSC, thereby proving the correctness of DurEC.

% To express how the auxiliary variables track progress, we annotate some lines of the algorithm with ``augmenting code'' that manipulate these variables.
% The auxiliary variables and the augmenting code for tracking them are simply a tool to facilitate the proof of correctness. 
% In particular, the augmenting code does not change any of the original program variables, thereby ensuring that the original algorithm's behavior is unaffected by the annotation.

\subsection{The Annotation}

The auxiliary variables can be broken into two groups: those associated with objects, and those associated with handles.
For each object $\O$, we introduce a single auxiliary variable:
\begin{itemize}
    \item
    \underline{$\O.\objstate$} stores the abstract state of the object $\O$, i.e., $\O.\objstate = (\O.\objstate.\seq, \O.\objstate.\val)$ is a state of the EC type.
\end{itemize}

\noindent
For each handle $\h$, we introduce the following auxiliary variables to track its ECSC operations:
\begin{itemize}
    \item 
    \underline{$\h.\args$} stores the arguments of $\h$'s ongoing ECSC operation (through crashes) when such an operation exists, and stores $\bot$ otherwise.

    \item
    \underline{$\h.\linearized$} is a boolean that stores whether $h$'s ongoing ECSC operation has linearized yet.

    \item
    \underline{$\h.\visible$} is a boolean that stores whether the ECSC operation had a visible effect on the object's state.

    \item
    \underline{$\h.\detval$} stores the value of $\h.\Last$ at the time that the ongoing ECSC operation was initiated if such as operation exists, and stores $\bot$ otherwise.
\end{itemize}
We present the annotated algorithm as Algorithm~\ref{alg:DurEC-Annotated}, where the annotations are underlined and \annotationColor\xspace in color.
The annotation below the ECSC method header initializes the auxiliary variables when the ECSC method is called.
The annotations at Lines 6, 12, and 21 reset the auxiliary variables as the operation returns. 
The most interesting annotation appears at Line 18, where upon a successful CAS, one or more ECSC operations linearize and $\objstate$ changes accordingly.
In particular, the ECSC operation of the handle in $\X.\hndl$ linearizes successfully, changing $\objstate$ to $(x.seq, \vh)$, and all the other pending ECSC operations linearize immediately (as unsuccessful operations).
Accordingly, $\X.\hndl$'s operation alone becomes visible.

\subsection{The Invariant}

We identify an invariant, which is strong enough to imply the durable linearizability and detectability of $\DurEC$ objects.
The invariant is stated in Figure~\ref{fig:durec-invariant}, and is informally described as follows.
TODO TODO TODO

\subsection{Proof of Durable Linearizability}

\begin{theorem}
    
\end{theorem}

we present the invariant for the DurEC algorithm.
We adopt the following conventions in the writing of the invariant:
\begin{enumerate}
    \item 
    The full invariant $I$ is the conjunction of the invariant parts $I_1$ through $I_{10}$ displayed in the figure, quantified over all handles $h$ and all DurEC objects $\O$.

    \item
    To facilitate the expression of the invariant and its proof, we augment the algorithm with auxiliary variables and some statements that manipulate only the auxiliary variables.
    The auxiliary variables do not affect the runs of the original algorithm, and are simply a tool to prove correctness \cite{}.    
    \end{enumerate}
The augmented algorithm and invariant in figures TODO and TODO.

Our augmentation is as follows.
\begin{enumerate}
    \item 
    We introduce four auxiliary variables per handle $h$:
    \begin{enumerate}
        \item 
        \underline{$h.operation$}: stores the name ($h.operation.name$) and arguments ($h.operation.args$) of the handle's current operation.
        Once the operation completes, $h.operation$ is $\bot$.
        \item
        \underline{}
    \end{enumerate}
\end{enumerate}

Augmented variables for a handle: 
{\em operation}, {\em linearized}, {\em successful}, {\em detval}

\begin{figure*}[!ht]

\fbox{\begin{minipage}\textwidth
Invariant statement is quantified over all DurEC handles $h$ and all DurEC objects $\O$

\begin{enumerate}
\item
% DurEC object's state is maintained in $Y$ at all times
$(state.seq, state.val) = (Y.seq, Y.val)$

\item
\begin{enumerate}
    \item 
    % At Lines 6 through 10, s holds the operation's sequence number argument
    $PC \in \{6, 7, 8, 9, 10, 11.*\} \implies (s = \mbox{operation}.args.seq)$

    \item
    % v and then h.Val hold the operation's value argument
    $PC \in \{6, 7\} \implies (v = \mbox{operation}.args.val)$

    \item
    $(PC \in \{8, 9, 10, 11.*\} \vee (PC \in \{20.*\} \wedge \mbox{operation}.name = \mbox{ECSC})) \implies (h.Val = \mbox{operation}.args.val)$
\end{enumerate}

\item
\begin{enumerate}
    \item 
    % The operation starts off as unlinearized.
    $PC = 6 \implies \neg \mbox{linearized}$
    
    \item
    $PC = 12 \implies \mbox{linearized}$    

    \item
    % Once past Line 6, an SC operation linearizes at the next update of Y
    $PC \in \{7, 8, 9, 10, 11.*\} \implies
     (\mbox{linearized} \iff Y.seq > s)
    $
\end{enumerate}


\item
\begin{enumerate}
    \item
    $\mbox{successful} \implies \mbox{linearized}$

    \item
    $\mbox{successful} \iff (h.Last > detval)$

    \item 
    % The SC operation cannot succeed until Line 10
    $PC \in \{6, 7, 8, 9, 10\} \implies \neg \mbox{successful}$

    \item
    $(PC \in \{11.*, 12\} \wedge \mbox{linearized}) \implies (r = \mbox{successful})$    
\end{enumerate}

\item 
\begin{enumerate}
    \item 
    % Y.seq is never ahead of X.seq
    $(X.seq = Y.seq) \vee (X.seq > Y.seq)$
    
    \item 
    $(X.seq = Y.seq) \implies (X.hndl.Last \ge X.seq)$
    
    \item 
    % If X is ahead of Y, the operation of X's handle must be an active, not yet linearized, SC operation that is executing the Forward method to change the object's sequence number from Y.seq and install the value h.Val 
    $(X.seq > Y.seq) \implies 
        ((X.hndl.PC \in \{13::18\})                \wedge
         (X.hndl.\mbox{operation} = \mbox{ECSC}(Y.seq, X.hndl.Val))    \wedge 
         (X.hndl.Last \le X.seq)                                       \wedge
         (X.hndl.\mbox{linearized} = \mbox{\em false}))
    $
\end{enumerate}

\item
\begin{enumerate}
    \item
    $PC \in \{7, 8, 9, 10, 11.*, 12\} \implies Y.seq \ge s$
    
    \item 
    $((PC \in \{9, 10\}) \wedge (X.seq = s)) \implies (h' = X.hndl)$
    
    \item 
    $((PC = 10) \wedge (X.seq = s)) \implies (s' > \max(h.Last, s))$
    
    \item 
    $PC \in \{11.*\} \implies (X.seq > s)$
\end{enumerate}

\item
\begin{enumerate}
    \item 
    $(h = X.hndl \wedge PC \in \{11.*, 12\}) \implies r$

    \item
    $((h \ne X.hndl) \wedge PC \in \{11.*, 12\} \wedge (X.seq > Y.seq = s)) \implies \neg r$
\end{enumerate}

\item
\begin{enumerate}
    \item 
    % If X.hndl has not completed the Forward method, then X.hndl.Last can't exceed X.seq. Furthermore, if X.hndl.Last < X.seq, then X.hndl has not gone past Line 15.
    $(h = X.hndl \wedge \mbox{operation}.name = \mbox{ECSC} \wedge PC \in \{16::18\}) \implies (h.Last = X.seq)$
    
    \item
    $X.hndl.Last < X.seq \implies (X.hndl.PC \in \{13::15\} \wedge \mbox{operation}.name = \mbox{ECSC})$
    
    % $   (((PC \in \{11.13::11.19, 20.13::20.19\}) \implies (h.Last \le X.seq)) \wedge
    %     ((h.Last < X.seq) \implies ((PC \in \{11.13::11.15\}) \vee (PC \in \{20.13::20.15\} \wedge \mbox{operation}.name = \mbox{ECSC}))))
    % $
\end{enumerate}

% \item
% % At any time past Line 6, Y.seq >= SC operation's sequence number.
% $((PC \in \{7, 8, 9, 10, 11.*\}) \vee (PC \in \{20.*\} \wedge \mbox{operation}.name = \mbox{ECSC}))  \implies (Y.seq \ge \mbox{operation}.args.seq)
% $

% \item
% $****** ((X.seq = Y.seq) \wedge (h = X.hndl) \wedge (PC \in \{11.*, 12, 20.*\})) \implies
%    (\mbox{linearized} \wedge \mbox{successful})
% $

\item
\begin{enumerate}
    \item 
    $(PC \in \{14,15\} \wedge ((x.hndl.Last < x.seq) \vee (h = X.hndl \wedge X.hndl.Last < X.seq))) \implies (x = X \wedge X.seq > Y.seq)$

    \item
    $(PC = 15 \wedge ((x.hndl.Last < x.seq) \vee (h = X.hndl \wedge X.hndl.Last < X.seq))) \implies (s' = x.hndl.Last)$
    
\end{enumerate}

\item
\begin{enumerate}
    \item 
    % No handle, including X.hndl, does unsafe stuff at Line 18
    $((PC \in \{14::18\}) \wedge ((Y.seq < x.seq) \vee (h = X.hndl \wedge Y.seq < X.seq))) \implies
     ((x = X) \wedge (X.hndl.Last = X.seq))
    $

    \item
    % No handle, including X.hndl, does unsafe stuff at Line 18
    $((PC \in \{17,18\}) \wedge ((Y.seq < x.seq) \vee (h = X.hndl \wedge Y.seq < X.seq))) \implies (v' = x.hndl.Val)
    $

    \item
    % No handle, including X.hndl, does unsafe stuff at Line 18
    $((PC = 18) \wedge ((Y.seq < x.seq) \vee (h = X.hndl \wedge Y.seq < X.seq))) \implies (y = Y)
    $
    
\end{enumerate}

% \item
% % X.hndl ensures progress at Lines 15 & 18
% $((h = X.hndl) \wedge (PC \in \{11.14, 11.15, 20.14, 20.15\}) \wedge (X.hndl.Last < X.seq)) \implies
%  (x = X)
% $

% \item
% $((h = X.hndl) \wedge (PC \in \{11.15, 20.15\}) \wedge (X.hndl.Last < X.seq)) \implies
%  ((x = X) \wedge (s' = x.hndl.Last))
% $

% \item
% $((h = X.hndl) \wedge (PC \in \{11.16, 11.17, 11.18, 20.16, 20.17, 20.18\}) \wedge (X.seq > Y.seq)) \implies
% (x = X)
% $

% \item
% $((h = X.hndl) \wedge (PC \in \{11.17, 11.18, 20.17, 20.18\}) \wedge (X.seq > Y.seq)) \implies
%  ((x = X) \wedge (v' = h.Val))
% $

% \item
% $((h = X.hndl) \wedge (PC \in \{11.18, 20.18\}) \wedge (X.seq > Y.seq)) \implies
%  ((x = X) \wedge (y = Y) \wedge (v' = h.Val))
% $

% \item
% % No handle, including X.hndl, does unsafe stuff at Line 15
% $((PC \in \{11.14::11.15, 20.14::15\}) \wedge (x.hndl.Last < x.seq)) \implies
%  ((x = X) \wedge (X.seq > Y.seq))
% $

% \item
% $((PC \in \{11.15, 20.15\}) \wedge (s' = x.hndl.Last) \wedge (s' < x.seq)) \implies
%  ((x = X) \wedge (X.seq > Y.seq))
% $

% \item
% % No handle, including X.hndl, does unsafe stuff at Line 18
% $((PC \in \{11.14::11.18, 20.14::18\}) \wedge (Y.seq < x.seq)) \implies
%  ((x = X) \wedge (X.hndl.Last = X.seq))
% $

% \item
% $
% ((PC \in \{11.17::11.18, 20.17::20.18\}) \wedge (Y.seq < x.seq)) \implies
%   (v' = X.hndl.Val)
% $

% \item
% $((PC \in \{11.18, 20.18\}) \wedge (y.seq < x.seq) \wedge (y = Y)) \implies
%  ((x = X) \wedge (X.hndl.Last = X.seq) \wedge (v' = X.hndl.Val))
% $
\end{enumerate}

\caption{Invariant for the DurEC Algorithm.}
\label{fig:durec-invariant}
\end{minipage}}

\end{figure*}

% Invariant statement is quantified over all DurEC handles $h$ and all DurEC objects $\O$

% % DurEC object's state is maintained in $Y$ at all times
% $(state.seq, state.val) = (Y.seq, Y.val)$

% % At Lines 6 through 10, s holds the operation's sequence number argument
% $(PC \in \{6, 7, 8, 9, 10, 11.*\}) \implies (s = \mbox{operation}.args.seq)$

% % v and then h.Val hold the operation's value argument
% $(((PC \in \{6, 7\}) \implies (v = \mbox{operation}.args.val)) \wedge
%   (PC \in \{8, 9, 10, 11.*, 12\} \vee (PC \in \{20.*\} \wedge \mbox{operation}.name = \mbox{ECSC})\implies (h.Val = \mbox{operation}.args.val)))
% $

% % The SC operation cannot succeed until Line 10
% $(PC \in \{6, 7, 8, 9, 10\}) \implies \neg \mbox{successful}$

% % The operation starts off as unlinearized.
% $(PC = 6) \implies \neg \mbox{linearized}$

% $PC \in \{7, 8, 9, 10, 11.*, 12\} \implies Y.seq \ge s$

% % Y.seq is never ahead of X.seq
% $(X.seq = Y.seq) \vee (X.seq > Y.seq)$

% % If X is ahead of Y, the operation of X's handle must be an active, not yet linearized, SC operation that is executing the Forward method to change the object's sequence number from Y.seq and install the value h.Val 
% $((X.seq > Y.seq) \wedge (h = X.hndl)) \implies 
%     ((PC \in \{11.13::11.18, 20.13::20.18\}) \wedge
%      (\mbox{operation} = \mbox{ECSC$(Y.seq, h.Val)$}) \wedge 
%      (h.Last \le X.seq) \wedge
%      (\mbox{linearized} = \mbox{\em false}))
% $

% $(X.seq = Y.seq) \implies (X.hndl.Last \ge X.seq)$

% $((PC \in \{9, 10\}) \wedge (X.seq = s)) \implies (h' = X.hndl)$

% $((PC = 10) \wedge (X.seq = s)) \implies (s' > \max(h.Last, s))$

% $PC \in \{11.*\} \implies (X.seq > s)$

% % If X.hndl has not completed the Forward method, then X.hndl.Last can't exceed X.seq. Furthermore, if X.hndl.Last < X.seq, then X.hndl has not gone past Line 15.
% $(h = X.hndl) \implies 
%    (((PC \in \{11.13::11.19, 20.13::20.19\}) \implies (h.Last \le X.seq)) \wedge
%     ((h.Last < X.seq) \implies ((PC \in \{11.13::11.15\}) \vee (PC \in \{20.13::20.15\} \wedge \mbox{operation}.name = \mbox{ECSC}))))
% $

% % At any time past Line 6, Y.seq >= SC operation's sequence number.
% $((PC \in \{7, 8, 9, 10, 11.*\}) \vee (PC \in \{20.*\} \wedge \mbox{operation}.name = \mbox{ECSC}))  \implies (Y.seq \ge \mbox{operation}.args.seq)
% $



% % Once past Line 6, an SC operation linearizes at the next update of Y
% $PC \in \{7, 8, 9, 10, 11.*\} \implies
%  (\mbox{linearized} \iff Y.seq > s)
% $


% $((X.seq = Y.seq) \wedge (h = X.hndl) \wedge (PC \in \{11.*, 12, 20.*\})) \implies
%    (\mbox{linearized} \wedge \mbox{successful})
% $

% $\mbox{successful} \implies \mbox{linearized}$

% $\mbox{successful} \iff (h.Last > detval)$

% $PC = 12 \implies \mbox{linearized}$

% $((PC \in \{11.*, 12\}) \wedge \mbox{linearized}) \implies (r = \mbox{successful})$

% % X.hndl ensures progress at Lines 15 & 18
% $((h = X.hndl) \wedge (PC \in \{11.14, 11.15, 20.14, 20.15\}) \wedge (X.hndl.Last < X.seq)) \implies
%  (x = X)
% $

% $((h = X.hndl) \wedge (PC \in \{11.15, 20.15\}) \wedge (X.hndl.Last < X.seq)) \implies
%  ((x = X) \wedge (s' = x.hndl.Last))
% $

% $((h = X.hndl) \wedge (PC \in \{11.16, 11.17, 11.18, 20.16, 20.17, 20.18\}) \wedge (X.seq > Y.seq)) \implies
% (x = X)
% $

% $((h = X.hndl) \wedge (PC \in \{11.17, 11.18, 20.17, 20.18\}) \wedge (X.seq > Y.seq)) \implies
%  ((x = X) \wedge (v' = h.Val))
% $

% $((h = X.hndl) \wedge (PC \in \{11.18, 20.18\}) \wedge (X.seq > Y.seq)) \implies
%  ((x = X) \wedge (y = Y) \wedge (v' = h.Val))
% $

% % No handle, including X.hndl, does unsafe stuff at Line 15
% $((PC \in \{11.14::11.15, 20.14::15\}) \wedge (x.hndl.Last < x.seq)) \implies
%  ((x = X) \wedge (X.seq > Y.seq))
% $

% $((PC \in \{11.15, 20.15\}) \wedge (s' = x.hndl.Last) \wedge (s' < x.seq)) \implies
%  ((x = X) \wedge (X.seq > Y.seq))
% $

% % No handle, including X.hndl, does unsafe stuff at Line 18
% $((PC \in \{11.14::11.18, 20.14::18\}) \wedge (Y.seq < x.seq)) \implies
%  ((x = X) \wedge (X.hndl.Last = X.seq))
% $

% $
% ((PC \in \{11.17::11.18, 20.17::20.18\}) \wedge (Y.seq < x.seq)) \implies
%   (v' = X.hndl.Val)
% $

% $((PC \in \{11.18, 20.18\}) \wedge (y.seq < x.seq) \wedge (y = Y)) \implies
%  ((x = X) \wedge (X.hndl.Last = X.seq) \wedge (v' = X.hndl.Val))
% $



==> proofs-old/invariant/DurECW-newproof.tex <==

\subsection{Proof of \DurECW}

\begin{lemma}
\mbox{ }
\begin{enumerate}
\item
$\pc \in \{9.*, 10\} \implies ((\s = \z.\seq) \wedge ((s < \Z.\seq) \vee (\z = \Z)))$
\item
$\pc \in \{13, 14\} \implies ((\w.\seq < \W.\seq) \vee (\w = \W))$
\item
$\pc \in \{19, 20\} \implies ((\zh.\seq < \Z.\seq) \vee (\zh = \Z))$
\end{enumerate}
\end{lemma}

\noindent
{\em Proof}: The check at Line~8 ensures that $\z.\seq = s$ at Lines 9.* and 10.
Furthermore, since $\Z.\seq$ increases each time $\Z$ is changed (by a successful ECSC on $\Z$ at Line~10 or Line~20), at Lines 9.* and 10, either $\Z$ is unchanged since Line~7 or $\Z.\seq$ has increased.
In the first case, $\zh = \Z$, and in the second case $\s = \z.\seq < \Z.\seq$.
Hence, we have the lemma.
\hfill $\blacksquare$


    
\item\label{iwri}
\begin{enumerate}
    
    \item
    % Install flips W.bit to make it differ from Z.bit.
    $\pc = 14 \implies (((\w.\bit = \z.\bit) \wedge (\w = \W)) \implies (\z.bit = \Z.bit))$
\end{enumerate}

\item\label{itra}
\begin{enumerate}

    \item
    % Move sets Z.val to W.val, and flips Z.bit to make it equal to W.bit.
    $\pc = 20 \implies 
    (((\wh.bit \neq \zh.bit) \wedge (\zh = \Z)) \implies (\wh = \W))$
\end{enumerate}
\end{enumerate}



Statement (1) follows from the check at Line~8 and the observation that whenever $\Z$ changes (because of a successful ECSC on $\Z$ at Line~10 or Line~20.

==> proofs-old/invariant/DurECW.tex <==

\begin{figure*}[!ht]

\fbox{\begin{minipage}\textwidth
For all DurECW handles $h$ and all DurECW objects $\O$, all of the following statements are true.

\begin{enumerate}

\item\label{iobj}
$(\self.\seq, \self.\val) = (\Z.\seq, \Z.\val)$

\item\label{icas}
    $\pc \in \{8, 9.*, 10\} \implies ((\s = \z.\seq) \wedge ((s < \Z.\seq) \vee (\z = \Z)))$
    
\item\label{iwri}
\begin{enumerate}
    \item
    $\pc \in \{13, 14\} \implies ((\w.\seq < \W.\seq) \vee (\w = \W))$
    \item
    % Install flips W.bit to make it differ from Z.bit.
    $\pc = 14 \implies (((\w.\bit = \z.\bit) \wedge (\w = \W)) \implies (\z.bit = \Z.bit))$
\end{enumerate}

\item\label{itra}
\begin{enumerate}
    \item
    $\pc \in \{19, 20\} \implies ((\zh.\seq < \Z.\seq) \vee (\zh = \Z))$
    \item
    % Move sets Z.val to W.val, and flips Z.bit to make it equal to W.bit.
    $\pc = 20 \implies 
    (((\wh.bit \neq \zh.bit) \wedge (\zh = \Z)) \implies (\wh = \W))$
\end{enumerate}


\item\label{iins}
$(\installer = \bot) \iff (\W.\bit = \Z.\bit)$

\item
$(\h = \installer) \implies 
        (\neg \linearized \wedge
        (\args = \W.val) \wedge
        \pc \in \{15.*, 16.*, 21-24, 25.*, 26.*\})$

\item
    $(\h = \installer \vee \hitchhiker(\h)) \implies
        ((\pc \in \{16.19, 16.20, 26.19, 26.20\} \implies (\zh = \Z)) \; \wedge$ \\
        \mbox{\hspace{2.1in}} $(\pc \in \{16.20, 26.20\} \implies (\wh = \W)))$

\item
    $((\h = \installer \vee \hitchhiker(\h)) \; \wedge$ \\
    \mbox{\hspace{0.03in}} $(\pc \in \{16.*, 26.*\} \vee (\pc \in \{15.19, 15.20, 25.19, 25.20\} \wedge \zh.seq < \Z.seq)))$ \\
    \mbox{\hspace{0.0in}} $\implies \forall \hh: ((\hh.\pc = 10) \implies ((\hh.\s < \Z.\seq) \; \wedge $ \\
    \mbox{\hspace{1.72in}} $ (\hh.\pc = 20) \implies ((\hh.\zh.\seq < \Z.\seq) \vee (\hh.\wh = \W)))$

\item\label{ilin}
\begin{enumerate}
    \item
    $\pc \in \{7, 9.*, 10\} \implies \neg \linearized$
    \item
    $\pc = 8 \implies (\linearized \iff ((\z.\val \neq \old) \vee (\old = \new)))$
    \item
    $\pc = 11 \implies (\linearized \wedge (\response = r))$
    \item
    $(\pc = 12) \implies \neg \linearized$
    \item
    $((\pc \in \{13, 14\} \wedge \w \neq \W) \vee (\pc = 14 \wedge \w.\bit \neq \z.\bit)) \; \implies $ \\
    \mbox{\hspace{1.1in}} $(\hitchhiker(\h) \vee \linearized)$
    \item
    $\pc \in \{15.*, 16.*\} \implies ((\h = \installer) \vee \hitchhiker(\h) \vee \linearized)$
    \item
    $(\pc = 17) \implies \linearized$
\end{enumerate}
    
\item\label{idet}
\begin{enumerate}
     \item
     $\visible \implies \linearized$
     \item
    $(\visible \vee (h = \installer)) \iff (\h.\Critical.\detval > \olddetval)$
\end{enumerate}

\end{enumerate}

\caption{Invariant for the DurECW Algorithm.}
\label{fig:durecw-invariant}
\end{minipage}}
\end{figure*}

==> proofs-old/invariant/DuraCAS.tex <==
\begin{figure*}[!ht]

\fbox{\begin{minipage}\textwidth
For all DuraCAS handles $h$ and for all DuraCAS objects $\O$, the conjunction of the following statements is true.

\begin{enumerate}

\item\label{iobj}
$\objstate = \Z.\val$

\item\label{icas}
\begin{enumerate}
    \item
    $\pc \in \{8, 9, 10.*, 11\} \implies ((\z.\seq < \Z.\seq) \vee (\z = \Z))$
    \item
    $\pc = 8 \implies ((\z.\val \neq \old) \implies (\linearized \wedge (\response = \false)) \; \wedge $ \\
    \mbox{\hspace{0.68in}} $((\z.\val = \old = \new) \implies (\linearized \wedge (\response = \true))))$
    \item
    $\pc = 9 \implies ((\z.\val = \old = \new) \implies (\linearized \wedge (\response = \true)))$
    \item
    $\pc \in \{10.*, 11\} \implies (\z.\val = \old \neq \new)$
    \item
    $(\old \neq \Z.val) \implies \linearized$
    \item
    $\pc = 12 \implies (\linearized \wedge (\response = \true))$
    \item
    $\pc = 13 \implies (\linearized \wedge (\response = \false))$
    \item
    $(\pc \in \{6, 7, 8, 9, 10.*, 11, 13\} \implies \neg \visible) \wedge (\pc = 12 \implies \visible)$
\end{enumerate}

\item\label{icas2}
{\bf If} $(((\pc \in \{7,8,9,10.*,11\} \wedge i=2) \vee (\pc \in \{8,9,10.*,11\} \wedge i=1 \wedge z \neq \Z) \wedge \neg \linearized)$, {\bf then}:

\begin{enumerate}
    \item
    $(\W.\bit \neq \Z.bit) \implies (\W.val \neq \Z.val)$
    \item
    $\forall \hh: (((\hh.\pc = 17) \wedge (\hh.\z.\bit = \hh.\w.\bit) \wedge (\hh.\w = \W)) \implies \hh.\v \neq \Z.val)))$
    \item
    $(\pc \in \{8,9,10.*,11\} \wedge i=2) \implies (z = \Z)$
\end{enumerate}
    
\item\label{iwri}
\begin{enumerate}
    \item
    $\pc \in \{14, 15, 16, 17\} \implies \neg \linearized$
    \item
    $\pc \in \{15, 16, 17\} \implies ((\w.\seq < \W.\seq) \vee (\w = \W))$
    \item
    % Install flips W.bit to make it differ from Z.bit.
    $\pc \in \{16, 17\} \implies (((\w.\bit = \z.\bit) \wedge (\w = \W)) \implies (\z.bit = \Z.bit))$
    \item
    $(\pc = 16 \wedge \z.\val = \v) \implies \linearized$
    \item
    $\pc = 17 \implies (v \neq \z.\val)$
\end{enumerate}

\item\label{itra}
\begin{enumerate}
    \item
    $\pc \in \{22, 23\} \implies ((\zh.\seq < \Z.\seq) \vee (\zh = \Z))$
    \item
    % Move sets Z.val to W.val, and flips Z.bit to make it equal to W.bit.
    $\pc = 23 \implies 
    (((\wh.bit \neq \zh.bit) \wedge (\zh = \Z)) \implies (\wh = \W))$
\end{enumerate}

\item\label{iins}
\begin{enumerate}
    \item
    $(\installer = \bot) \iff (\W.\bit = \Z.\bit)$
    \item
    {\bf If} $\installer \neq \bot$, {\bf then:}
    \begin{enumerate}
        \item
        $\neg \installer.\linearized$
        \item
        $\installer.\pc \in \{18.*, 19.*, 24, 25, 26, 27, 28.*, 29.*\}$
        \item
        $\installer.\args = \W.val$
        \item
        $\installer.\pc \in \{19.22, 19.23, 29.22, 29.23\} \implies (\installer.\zh = \Z)$
        \item
        $\installer.\pc \in \{19.23, 29.23\} \implies (\installer.\wh = \W)$
    \end{enumerate}
    \item
    {\bf If} $((\installer \neq \bot) \wedge (\installer.\pc \in \{19.*, 29.*\} \vee (\installer.\pc \in \{18.22, 18.23, 28.22, 28.23\} \wedge \installer.\zh.seq < \Z.seq)))$, {\bf then} for all handles $\hh$:
    \begin{enumerate}
    \item
    $(\hh.\pc = 11) \implies (\hh.\z.\seq < \Z.\seq)$
    \item
    $(\hh.\pc = 23) \implies ((\hh.\zh.\seq < \Z.\seq) \vee (\hh.wh = \W))$
    \end{enumerate}
\end{enumerate}

\item\label{idet}
\begin{enumerate}
     \item
     $\op.\name \in \{\cas, \writ\} \implies (\visible \implies \linearized)$
     \item
    $\op.\name \in \{\cas, \writ\} \implies $ \\
    \mbox{\hspace{0.4in}} $((\visible \vee (h = \installer)) \iff (\DurEC.\Detect{\h.\Critical} > \detval))$
\end{enumerate}

\end{enumerate}

\caption{Invariant for the DuraCAS Algorithm.}
\label{fig:duracas-invariant}
\end{minipage}}
\end{figure*}

==> spec/Spec-DetCAS-2022.tex <==
\section{Durable and Detectable CAS Objects}

In this section, we describe the specifications of the {\em CAS/Write object}, abbreviated {\em CASW object}, and design an adaptive and linear space and constant time algorithm that implements a durable and detectable version of CAS using the DetEC objects described in Section ????.


\subsection{Specification of a CASW object}

A CASW object $\O$'s state consists of a single field $\O.value$,
and the object supports the following three operations.
(Like the EC object described above, the first argument of an operation of a CASW object is also {\em Proc\_Info}.)

\begin{itemize}
\item
Read$(\mbox{Proc\_Info } h)$: returns $O.value$.
\item
CAS$(\mbox{Proc\_Info } h, \mbox{Value } old, \mbox{Value } new)$: if $\O.value = old$, the operation sets $\O.value$ to $new$ and returns {\em true}; otherwise, the operation returns {\em false} without affecting the state.

We call a CAS operation {\em successful} if it changes the object's state, and {\em unsuccessful} or {\em failed} otherwise. 
\item
Write$(\mbox{Proc\_Info } h, \mbox{Value } val)$: changes the $\O.value$ to $val$.
\end{itemize}

\subsubsection{Durable CASW objects}

A durable CASW object supports an additional method, {\em Recover}$(\mbox{Proc\_Info } h)$. As always, if a process crashes while executing any operation or method on an EC object $\O$ (including the recover method), the process is required to execute $\O$.Recover$(h)$ when it restarts (and, more specifically, before it may invoke any other methods or operations).

\subsubsection{Durable and Detectable CASW objects}

Suppose that a process $p$ crashes during a Read operation or a CAS or Write operation that took effect but is unsuccessful.
Once $p$ restarts and executes the recover method to completion, it is harmless for $p$ to repeat the Read, CAS, or Write method.
Thus, the only operations that need detection are successful CAS and Write operations.
Hence, we require the Detectable and Durable CASW class (called DetCAS) to support a method {\em Detect}$(\mbox{Proc\_Info } h)$ with the following property:

% \begin{itemize}
% \item 
% \underline{EC Detection Property}: Suppose that a process $p$ executes an operation $\alpha$ on an EC object ($\alpha$ can be any of ECLL, ECVL, or ECSC).
% Furthermore, suppose that $p$ also executes {\em Detect}$(h)$ immediately before invoking $\alpha$ and immediately after completing $\alpha$,\footnote{By ``immediately'' we mean that the process does not execute any other operations on EC objects between the first call to {\em Detect} and $\alpha$'s invocation nor between $\alpha$'s completion and the second call to {\em Detect}.} and the Detect method returns $r_1$ and $r_2$ for the two calls.
% Then, $r_1 \neq r_2$ if and only if $\alpha$ is a successful ECSC operation.
% \end{itemize}

% \subsection{DurEC: the Durable and Detectable EC Class}

% We design the class {\em DurEC} that makes it possible for processes to create and operate on durable and detectable EC objects (henceforth, DurEC objects).
% The class implements all of the operations (ECLL, ECSC, ECVL) and methods (Recover and Detect), and additionally has the following key features:

% \begin{enumerate}
% \item
% Initially, no DurEC objects exist.
% Processes create new objects as and when they need them
% (via the class constructor method).
% \item
% Initially, the ``user set''---the set of processes that may access DurEC objects---is also empty.
% Only those processes in the system that wish to create or access the DurEC objects add themselves to the user set.
% Specifically, the class provides a method---{\sc CreateHandle}$()$, which a process calls when it first wishes to become a user.
% The method creates and returns a ``handle'', which is simply a record where the algorithm maintains some relevant information.
% Anytime the process calls an ECLL, ECSC, or any other operation, it passes its handle as an argument to the operation
% (the handle is what we have called ``Proc\_Info'' thus far).
% \item
% Once a process creates a handle, it can use that same handle for any of its operations and methods on any of the DurEC objects.
% Thus, a process' handle is not specific to any DurEC object, and is good for the entire class of objects.
% (Consequently, {\sc CreateHandle} is a static method, in the parlance of Java.)
% \item
% Each object and each handle takes only constant space.
% \end{enumerate}

% The first two features are crucial for achieving adaptive space complexity---that the space complexity depends only on the actual number $m$ of objects needed in the run and only on the number $n$ of processes that truly need to access these objects (as opposed to conservative upper bounds on the number of objects and processes).

% The third and fourth features ensure that the space complexity is $O(m+n)$ (instead of, for instance, $O(mn)$).

% Furthermore, the design does not use process IDs and does not impose any limit on the number of processes, and thus supports an arbitrary number of processes of arbitrary names.

% \subsection{DurEC: Intuitive description of the algorithm}

% Our algorithm---the DurEC class---is presented in Figure~\ref{}.


% \subsection{DurEC: Proof of correctness}













 


==> spec/Spec-DetEC-2022.tex <==
% We define the Durable, Detectable, External Context LL/SC (DetEC) object.

% A DetEC object $\O$ = (context, value) where both context and value are integer fields, a context field and a value field and supports five methods specified as follows:
% \begin{itemize}
%     \item $\CLL{\mbox{\em process\_info}}$ -- returns ($\O$.context, $\O$.value)
%     \item $\CVL{\mbox{\em process\_info}, \textbf{int} \: con}$ -- If con equals $\O$.context, returns $\true$, else, returns $\false$.
%     \item $\CSC{\mbox{\em process\_info}, \textbf{int} \: con, \textbf{int} \: val}$ -- If con = $\O$.context, sets $\O$.value = val and $\O$.context = c, where c is a never before seen context.
%     \item $\Recover{\mbox{\em process\_info}}$ -- 
%     \item $\Detect{\mbox{\em process\_info}}$ -- 
% \end{itemize}

\section{Durable and Detectable External Context LL/SC Objects}

In this section, we define an {\em External Context LL/SC object}, abbreviated {\em EC object}, and design an adaptive and linear space and constant time algorithm that implements durable and detectable version of these EC objects using regular (non-durable) Read/CAS objects (that do not support write operations).
These objects are the backbone for the algorithms of the later sections that efficiently implement durable and detectable CAS/Write and LL/SC/Write objects.

\subsection{Specification of an EC object}

An EC object $O$'s state consists of $O.context$ and $O.value$,
and the object supports the following three operations.
(It is common to let the first argument of an operation be {\em Proc\_ID} --- the ID of the process executing the operation, but we let it be more general and call it  {\em Proc\_Info}, which can be a reference to where info about the process can be found.)

\begin{itemize}
\item
ECLL$(\mbox{Proc\_Info } h)$: returns $(O.context, O.value)$.
\item
ECSC$(\mbox{Proc\_Info } h, \mbox{Context } c, \mbox{Value } v)$: if $O.context = c$, the operation sets $O.value$ to $v$, changes $O.context$ to a context that was never the object's context in the past, and returns {\em true}; otherwise, the operation returns {\em false} without affecting the state.

We call an ECSC operation {\em successful} if it changes the object's state, and {\em unsuccessful} or {\em failed} otherwise. 
\item
ECVL$(\mbox{Proc\_Info } h, \mbox{Context } c)$: returns {\em true} if $O.context = c$, and returns {\em false} otherwise.
\end{itemize}

\subsubsection{Durable EC objects}

A durable EC object supports an additional method, {\em Recover}$(\mbox{Proc\_Info } h)$. As always, if a process crashes while executing any operation or method on an EC object $O$ (including the recover method), the process is required to execute $O$.Recover$(h)$ when it restarts (and, more specifically, before it may invoke any other methods or operations).

\subsubsection{Durable and Detectable EC objects}

Suppose that a process $p$ crashes during an ECLL or ECVL operation, or during an ECSC operation that took effect but is unsuccessful.
Once $p$ restarts and executes the recover method to completion, it is harmless for $p$ to repeat the ECLL, ECVL, or the ECSC method.
Thus, the only operation that needs detection is a successful ECSC operation.
Hence, we require the Detectable and Durable EC class to support a method {\em Detect}$(\mbox{Proc\_Info } h)$ with the following property:

\begin{itemize}
\item 
\underline{EC Detection Property}: Suppose that a process $p$ executes an operation $\alpha$ on an EC object using a handle $h$ ($\alpha$ can be any of ECLL, ECVL, or ECSC).
Furthermore, suppose that $p$ also executes {\em Detect}$(h)$ immediately before invoking $\alpha$ and immediately after completing $\alpha$,\footnote{By ``immediately'' we mean that the process does not execute any other operations on EC objects between the first call to {\em Detect} and $\alpha$'s invocation nor between $\alpha$'s completion and the second call to {\em Detect}.} and the Detect method returns $r_1$ and $r_2$ for the two calls.
Then, $r_1 \neq r_2$ if and only if $\alpha$ is a successful ECSC operation.
\end{itemize}

\subsection{The Algorithm}

We design an algorithm that makes it possible for processes to create and operate on durable and detectable EC objects (henceforth, DurEC objects).
The algorithm implements the DurEC class, which has methods for the ECLL, ECSC, and ECVL operations, and for Recover and Detect.
Besides ensuring durable linearizability and detectability, this algorithm as well as the other two algorithms of this paper enable processes to dynamically join and create objects, and ensure adaptive and linear space complexity.
In the rest of this section, we first introduce the methods that make these properties possible.
We then present the algorithm, along with an intuitive description of how the algorithm works.
We end the section with a proof of the algorithm's correctness.


\vspace{0.1in}
\noindent
{\bf 2.2.1 \mbox{\hspace{0.03in}}Methods for dynamic creation of objects and joining of processes}

The DurEC class supports the following two methods for dynamic creation of objects and joining of processes.

\begin{itemize}
\item
The constructor method of the DurEC class enables dynamic creation of objects.
Thus, there are no DurEC objects initially,
and processes create new objects as and when they need them by calling the constructor.

\item
The DurEC class implements a {\sc CreateHandle}$()$ method for processes to gain the right to create and access DurEC objects.
More specifically, the ``user set''---the set of processes that may create or access DurEC objects---is initially empty.
Whenever a process wishes to become a user, it calls {\sc CreateHandle}$()$, which creates and returns a ``handle''.
A handle is simply a record where the algorithm maintains some relevant information.
Anytime a process calls an ECLL, ECSC, or any other operation or method, it is required to pass a handle (that it previously created) as an argument to the operation
(the handle is what we have called ``Proc\_Info'' thus far).
\end{itemize}

These two methods ensure that the space used by the algorithm depends only on the actual number $m$ of objects needed in the run and only on the number $n$ of processes that truly need to access these objects (as opposed to conservative upper bounds on the number of objects and processes).

A noteworthy feature is that, once a process creates a handle, it can use that same handle for any of its operations and methods on any of the DurEC objects.
Thus, a process' handle is not specific to any DurEC object, and is good for the entire class of objects.
(Consequently, {\sc CreateHandle} is a static method, in the parlance of Java.)


%Our methods do not use process IDs or require that the process IDs should be from any specific set (like $\{1, \ldots, N\}$ or even the set of integers).Consequently, our design supports an arbitrary number of processes of arbitrary names.

\subsection{The algorithm and an intuitive description of how it works}

Our algorithm implements the DurEC class and is presented in Figure~\ref{}.


\subsection{Proof of the algorithm's correctness}













 

